FG-OrIU: Towards Better Forgetting via Feature-Gradient Orthogonality for Incremental Unlearning

Incremental unlearning (IU) is critical for pre-trained models to comply with sequential data deletion requests, yet existing methods primarily suppress parameters or confuse knowledge without explicit constraints on both feature and gradient level, resulting in \textit{superficial forgetting} where residual information remains recoverable. This incomplete forgetting risks security breaches and disrupts retention balance, especially in IU scenarios. We propose FG-OrIU (\textbf{F}eature-\textbf{G}radient \textbf{Or}thogonality for \textbf{I}ncremental \textbf{U}nlearning), the first framework unifying orthogonal constraints on both features and gradients level to achieve deep forgetting, where the forgetting effect is irreversible. FG-OrIU decomposes feature spaces via Singular Value Decomposition (SVD), separating forgetting and remaining class features into distinct subspaces. It then enforces dual constraints: feature orthogonal projection on both forgetting and remaining classes, while gradient orthogonal projection prevents the reintroduction of forgotten knowledge and disruption to remaining classes during updates. Additionally, dynamic subspace adaptation merges newly forgetting subspaces and contracts remaining subspaces, ensuring a stable balance between removal and retention across sequential unlearning tasks. Extensive experiments demonstrate the effectiveness of our method.

==> sec/111.tex <==
\section{Introduction}
\label{sec:intro}

In recent years, \textit{pre-training with fine-tuning} \cite{zhang2025parameter,han2024parameter,xu2023parameter}, has garnered significant attention \cite{dosovitskiy2020image,radford2021learning,liu2024improved,jia2022visual,zhou2022learning,zhou2022conditional,tu2024texttoucher}. However, large-scale datasets, which include open-source, internet, and synthetic data, often contain harmful information and potential personal data leaks. To address this issue, the `right to be forgotten' (RTBF \cite{rosen2011right,regulation2018general}) has been introduced to safeguard user privacy by granting individuals the right to request the removal of personal information. These deletion requests not only require the removal of relevant data from the pre-training dataset but also necessitate modifications to the pre-trained models (PTMs) \cite{qin2024machine,cao2015towards,guo2019certified,shi2025redefining,bonato2024retain,foster2024fast,chundawat2023can,huang2024unified,bourtoule2021machine,shaik2024exploring,xu2024machine}. Moreover, as deletion requests typically emerge over time, handling them incrementally better fulfills the needs of real-world scenarios \cite{cheng2024remaining,zhao2025practical,zhao2024continual,wang2024has,gao2024practical,liu2022continual,chatterjee2024unified,kumaraveluuncle,chen2023unlearn,jang2022knowledge,grimes2024gone}.


Given the identified necessities, researchers have introduced the Machine Unlearning (MU) task for PTMs \cite{xu2024machine,shaik2024exploring,bourtoule2021machine,guo2019certified,nguyen2022survey}. Prior works primarily focus on addressing the computer vision classification task \cite{qin2024machine,jia2023model}, aiming to make PTMs forget specific classes ($\mathbf{D_f}\downarrow$) while retaining irrelevant class ($\mathbf{D_r}\uparrow$). Typically, existing MU methods can be categorized into \textit{exact MU} \cite{bourtoule2021machine} and \textit{approximate MU} \cite{choi2023towards,perifanis2024sftc,foster2024fast,graves2021amnesiac,kurmanji2023towards,chundawat2023can}. Achieving exact MU  requires retraining the model on a dataset that excludes the forgetting samples, which serves as a golden standard but is impractical due to the prohibitive computational cost for PTMs. In this study, we primarily focus on more efficient approximate MU (hereafter referred to as MU).




A seemingly effective approach is to directly set the parameters corresponding to the forgetting classes in the MLP head to zero. However, this crude method merely removes the decision boundary while leaving the underlying features intact, meaning the forgetting effect can be easily and completely recovered. Researchers have termed this \textit{pseudo forgetting} \cite{zhao2025practical, zhao2024continual, huang2024unified, cheng2024remaining}. Thus, prior works in MU have focused on forgetting within the backbone rather than the MLP head, primarily addressing the final output, which can be broadly categorized into \textit{parameter suppression} and \textit{knowledge confusion}. The former suppresses the core parameters that are highly responsible for predicting the forgetting classes \cite{yan2022arcane, fan2023salun, goel2022towards, foster2024fast}, while the latter obfuscates the prediction through random labeling or distillation with a poor teacher model \cite{kurmanji2023towards, graves2021amnesiac, chundawat2023can, golatkar2020eternal}. \textcolor{red}{However, these methods do not impose adequate constraints on the feature representations in the intermediate layers of the PTM, leading to a \textit{tug-of-war}, where one side’s gain is equivalent to the other side’s loss.} Furthermore, empirical results shown in Figure \ref{fig:figure1} further indicate that existing MU methods, due to the absence of explicit constraints at the feature level, only weaken the unlearned model’s feature extraction capabilities, making the degraded features less effective. Specifically, we use Deep Image Prior (DIP) \cite{ulyanov2018deep} to reconstruct the features extracted by the unlearned PTM through different MU methods. Surprisingly, the features can still reconstruct a blurred image, indicating the persistence of residual information. Therefore, although these methods can achieve a significant reduction in classification accuracy on the forgetting classes, \textbf{they essentially only achieve incomplete forgetting}. Since the extracted features of the forgetting data are merely degraded and not entirely removed, when freezing its backbone and retraining a new MLP head, the forgetting effect can still be partially restored in most cases, which aligns with the observations of \cite{zhao2025practical, zhao2024continual}.

\begin{table}[t]
\centering
\caption{\textit{Position, Capability, Complete, and Recover} refers to, where the forgetting occurs, the feature capability of the unlearned model, whether the forgetting is thorough, and whether the forgetting effect can be restored, respectively.}
\vspace{-2mm}
\label{tab:tab1}
\resizebox{\columnwidth}{!}{ % Resize the table to fit the text width
\small
\begin{tabular}{l|llll}
\hline
 & \textit{Position} & \textit{Capability} & \textit{Complete} & \textit{Recover} \\
\hline
\multirow{2}{*}{Prior works} & MLP  & Intact & No & Yes \\
% \hline
& Output & Degraded & No & Partial \\
\hline
\textbf{Ours} & \textbf{Feature} & \textbf{Eliminated}  & \textbf{Yes} & \textbf{No} \\
\hline
\end{tabular}
}
\vspace{-6mm}
\end{table}

Incomplete forgetting not only introduces potential privacy and security concerns, as personal information has not been thoroughly erased \cite{tu2025sdwv, chin2023prompting4debugging}, but also disrupts the balance between removal and retention. The degraded features are likely to become entangled with the features from the remaining data \cite{qin2024machine, cheng2024remaining}, thereby negatively impacting the performance of the remaining data. Moreover, in practical unlearning scenarios, the PTM may face deletion requests that arrive sequentially, requiring multiple executions of MU methods. This exacerbates the dilemma between forgetting and remaining, leading to severe deterioration in the PTM \cite{cheng2024remaining, wang2024has, zhao2025practical, zhao2024continual, gao2024practical, jang2022knowledge}.








In summary, to strictly meet the deletion request from individuals, the MU approach should thorough eliminate the unlearned PTM’s capability to extract features related to the forgetting data, thereby \textbf{achieving complete forgetting that cannot be recovered}. In Table \ref{tab:tab1}, we compare our methods with prior works across four characteristics.



In this paper, we propose \textbf{FEAST} (\textbf{F}eature \textbf{E}liminate via \textbf{A}daptive \textbf{S}ubspace \textbf{T}ransformation), a holistic framework designed to precisely eliminate unwanted features while maintaining a robust balance between removal and retention. FEAST consists of three stages: {Disentangled Feature Subspace}, {Bidirectional Feature Disturbing-Denoising}, and {Dynamic Subspace Adaptation}. In {Disentangled Feature Subspace}, we apply Singular Value Decomposition (SVD) to the feature matrices of both forgetting data ($\mathbf{D_{f}}$) and remaining data ($\mathbf{D_{r}}$), yielding two disentangled feature subspaces: an unwanted feature subspace ($\mathcal{S}_{f}$), which captures features to be forgotten, and a desired feature subspace ($\mathcal{S}_{r}$), which preserves features to be retained. In {Bidirectional Feature Disturbing-Denoising}, we freeze the PTM backbone and introduce lightweight LoRA modules for efficient updates. We impose a bidirectional constraint strategy to ensure effective removal and retention. Specifically, in \textit{Disturbing for Forgetting} during the forward pass, we enforce the features of $\mathbf{D_{f}}$ deviate from $\mathcal{S}_{f}$ through orthogonality constraints, thus breaking their correlation with unwanted features; meanwhile, in \textit{Denoising for Retention}, we ensure that the features of $\mathbf{D_{r}}$ align with $\mathcal{S}_{r}$ by minimizing the projection residual, effectively filtering out interference from unwanted features. Then, in the backward pass, we impose \textit{Disturbing and Denoising} on the gradients sequentially. The former adjusts the gradients by projecting them onto $\mathcal{S}_{f}$, forcing updates in a direction that maximally perturbs parameters most critical for unwanted features. The latter projects the gradients onto the complementary space of $\mathcal{S}_{r}$, ensuring that updates occur in directions that prevent contamination of retained features. In {Dynamic Subspace Adaptation}, FEAST handles sequential deletion requests by dynamically updating both disentangled feature subspaces through the expansion of $\mathcal{S}_{f}$ and the contraction of $\mathcal{S}_{r}$. 


\textbf{Our main contributions are threefold:}
\setlength{\leftmargini}{8pt} 

\begin{itemize}
  % \vspace{-4mm}
\item We reveal that existing MU methods only achieve \textit{feature degradation} rather than complete forgetting, as their partial feature suppression leaves residual information recoverable.

\item We propose the first framework to achieve \textit{feature elimination} via adaptive subspace transformation, ensuring irreversible forgetting while maintaining retention robustness.

\item Extensive experiments validate our method’s superiority in both static and dynamic scenarios.

\end{itemize}









\subsubsection{Feature Orthogonal Projection} 
Inspired by \cite{tu2025sdwv,yoon2024safree}, for forgetting classes, achieving thorough removal at the feature level requires that the features generated by the unlearned model, $\mathcal{M}_{\theta}$, deviate as much as possible from the feature subspace $\mathcal{S}_{f}$. Meanwhile, we aim to ensure that the unlearned model's feature subspace for remaining classes aligns with $\mathcal{S}_{r}$. The orthogonality constraint between $\mathcal{S}_{f}$ and the unlearned features serves as a critical mechanism for facilitating class-specific forgetting: under a fixed classification head, features orthogonal to the original subspace $\mathcal{S}_{f}$ induce maximal perturbations in class logits, as the inner product between orthogonal vectors diminishes to zero. This forces the unlearned model to suppress discriminative patterns associated with forgetting classes in its intermediate representations. To do so, we propose the following two propositions, along with its regularization constraints.
% \begin{tcolorbox}[colback=gray!10, colframe=white, sharp corners, boxrule=0pt]\small
\vspace{-2mm}
\begin{proposition}[Feature Orthogonal Projection for Forgetting (FOP-F)]
\label{proposition_1}
For a batch of forgetting samples from $\mathbf{D_{f,i}}$, let $\bm{h}_f^{l}$ denote the $l$-th layer features gained with the unlearned model $\mathcal{M}_{\theta}$.
For complete forgetting, we enforce:
\begin{align}
\bm{h}_f^{l} \perp \mathcal{S}_{f,i}^l \quad \Rightarrow \quad \min ||\bm{h}_f^{l} - \mathbf{P}_{f}^{l} \bm{h}_f^{l}||_F^2
\end{align}
where $\mathbf{P}_{f}^{l}=\mathbf{B}_{f,i}^{l}{(\mathbf{B}_{f,i}^{l})}^{\top}$ is the projection matrix for remaining subspace $\mathcal{S}_{f,i}^{l}$ and $||\cdot||_{F}^{2}$ is the F-norm.
\end{proposition}
Proposition \ref{proposition_1} ensures that the features of $\mathbf{D_{f,i}}$ gained from the unlearned model $\mathcal{M}_{\theta}$ lie outside the original feature subspace gained from $\mathcal{M}$, erasing the unwanted information. Thus, we define the {fop-f loss}:
\begin{align}
\label{loss:L_fop-f}
\mathcal{L}_{fop-f} = \sum_{l=1}^{m} ||\bm{h}_f^{l}- \mathbf{P}_{r}^{l}\bm{h}_f^{l}||_F^2.
\end{align}

For remaining classes, we follow previous works and apply the standard cross-entropy loss by constraining the model’s final output, as follows:
\begin{align} 
\label{loss:L_ce}
\mathcal{L}_{ce} = \mathcal{L}(\mathcal{X}_{\mathbf{D}_{r,1}}, \mathcal{Y}_{\mathbf{D}_{r,1}}), 
\end{align}
where $\mathcal{L}$ denotes the cross-entropy loss function. In addition, we also propose applying explicit constraint at the feature level for the remaining data to better preserve the desired information.
% \begin{tcolorbox}[colback=gray!10, colframe=white, sharp corners, boxrule=0pt]\small
\begin{proposition}[Feature Orthogonal Projection for Remaining (FOP-R)]
\label{proposition_2}
For a batch of remaining samples from $\mathbf{D_{r,i}}$, let $f_{l}({x_{r}})$ denote the $l$-th layer features gained with the unlearned model $\mathcal{M}_{\theta}$. For better preservation, we maintain feature fidelity through:
\begin{align}
\min ||f_l(x_r) - \mathbf{P}_{r}^{l} f_l(x_r)||_F^2
\end{align}
where $\mathbf{P}_{r}^{l}=\mathbf{B}_{r,i}^{l}{(\mathbf{B}_{r,i}^{l})}^{\top}$ is the projection matrix for $\mathcal{S}_{r,i}^{l}$.
\end{proposition}

% $f_{l}({x_{r}})$ should align closely with the feature subspace $\mathcal{S}_{r,i}^{l}$ spanned by the original model $\mathcal{M}$'s features. The optimal condition is minimal projection residual: $||f_{l}({x_{r}}) - f_{l}({x_{r}})\mathbf{P}_{l}||_F^2 = 0$.
% \end{proposition}
% % \end{tcolorbox}

Based on Proposition \ref{proposition_2}, the features of $\mathbf{D_{r,i}}$ gained from the unlearned model $\mathcal{M}_{\theta}$, align with the orignal feature subspace gained from $\mathcal{M}$, maintaining the better preservation. We then draw the following fop-r loss:
\begin{align}
\label{loss:L_fop-r}
\mathcal{L}_{fop-r} = \sum_{l=1}^{m} ||f_{l}({x_{r}}) - \mathbf{P}_{r}^{l}f_{l}({x_{r}})||_F^2.
\end{align}

Finally, the total loss is:
\begin{align}
\label{eq:total_loss}
\mathcal{L}_{total} = \mathcal{L}_{ce} + \lambda_1 \mathcal{L}_{fop-f} + \lambda_2 \mathcal{L}_{fop-r},
\end{align}
where $\lambda_1$, $\lambda_2$ are the coefficients during training.






\subsubsection{Gradient Orthogonal Projection} 
To prevent parameter updates from reintroducing forgotten knowledge while preserving retained features, we design a gradient correction mechanism inspired by gradient projection techniques in multi-task learning \cite{yu2020gradient} and continual learning \cite{zhao2023rethinking,saha2021gradient}. Given the raw gradient $\bm{g_{l}}$ at layer $l$, we apply the following modifications:
\begin{align}
\label{eq:original approx unlearn steepest descent}
&\hat{\bm{g_{l}}}=\bm{g_{l}} - {\bm{g'_{l}}} - {\bm{g''_{l}}}\\
&=\bm{g_{l}} - \underbrace{\bm{g_{l}}(\bm{I} - \mathbf{B}_{f,i}^{l}{(\mathbf{B}_{f,i}^{l})}^{\top})}_{(term1: gop-f)} - \underbrace{\bm{g_{l}}\mathbf{B}_{r,i}^{l}{(\mathbf{B}_{r,i}^{l})}^{\top}}_{(term2:gop-r)}, \nonumber
\end{align}

\noindent
\textbf{Term (gop-f)} Removing the components of $\bm{g'_{l}}$ that are orthogonal to $\mathcal{S}_{f,i}^{l}$ not only amplifies updates focusing on directions most critical for encoding forgetting class features, but also blocks parameter updates that could re-introduce removed knowledge.

\noindent
\textbf{Term (gop-r)} We aim to ensure that forgetting specific classes does not affect the remaining classes. Formally, for the unlearned model $f_{\mathcal{M}_{\theta}}$ and $\bm{x}_{r}$ from the remaining classes $\mathbf{D_{r,i}}$, the following equation holds: $f_{\mathcal{M}_{\theta}}(x_{r})=f_{\mathcal{M}}(x_{r})$. Specifically, we consider the input and output of layer $l$ as follows:
\begin{align}
\label{eq10}
\bm{W}_{l}\bm{x_{r}} + \Delta \theta_{l} \bm{x_{r}} &= \bm{W}_{l} \bm{x_r} \\
\Delta \theta_{l} \bm{x_{r}} &= \bm{0}
\end{align}
where $\Delta \theta_{l}$ represents the change in the LoRA parameters inserted at layer $l$, which corresponds to its gradient. $\bm{W}_{l}$ is the parameter at layer $l$ from the pre-trained model, and these parameters remain frozen during unlearning.

Eq. (\ref{eq10}) indicates that if the update direction of the parameters, \ie, the gradient of the trainable LoRA parameters, lies in the complementary space of $\mathcal{S}_{r,i}^{l}$, \ie, $\bm{g_{l}} \perp \mathcal{S}_{r,i}^{l}$, then $\Delta \theta \bm{x_{r}} = \eta \bm{g_{l}}\theta \bm{x_{r}} = \bm{0}$ (where $\eta$ is the learning rate), ensuring that the unlearned model’s performance on the remaining classes is not affected. Therefore, we further refine the gradient by removing its components along $\mathcal{S}_{r,i}^{l}$.



Finally, modified gradient $\hat{\bm{g}_{l}}$ serves the real gradient for parameter updates at the layer $l$.




==> sec/7_ack.tex <==
\vspace{-2mm}
\section{Acknowledgement}
\label{sec:acknowledgement}
\vspace{-2mm}
This work was supported in part by National Natural Science Foundation of China under Grant 62402430, 62206248, 62476238, Zhejiang Provincial Natural Science Foundation of China under Grant LQN25F020008, and Aeronautical Science Foundation of China 20240048076001. 

==> sec/app.tex <==
% This decomposition enables targeted manipulation of feature representations, ensuring effective removal of unwanted knowledge while maintaining the integrity of retained knowledge.
% Given a PTM, $\mathcal{M}$, with consecutive operations, $f_\mathcal{M}(\cdot) = \{f_{i}(\cdot)\}^{m}_{i=1}$. We construct a representation matrix $\bm{R}_{f,i}^{l}=\left[\bm{x}^{l}_{1,i},\dots,\bm{x}^{l}_{n_{f_{i}},i}\right] \in \mathbb{R}^{n_{f_{i}} \times d}$ at each layer $l$, where columns correspond to representations of $n_{f_{i}}$ samples from the remaining classes $\mathbf{D_{f,i}}$, and $d$ is the output dimension. Singular Value Decomposition (SVD) is applied to $\bm{R}_{f,i}^{l}=\bm{U}_{f,i}^{l}\bm{\Sigma}_{f,i}^{l}(\bm{V}_{f,i}^{l})^{T}$, followed by its $k$-rank approximation ${(\bm{R}_{f,i}^{l})}_{k}$ satisfying $||(\bm{R}_{f,i}^{l})_{k}||_{F}^{2} \geq \epsilon ||\bm{R}_{f,i}^{l}||_{F}^{2}$ for a threshold $\epsilon$. The subspace $\mathcal{S}_{f,i}^{l} = \text{span} \left\{\bm{B}_{f,i}^{l}\right\}$ is defining using the first $k$ vectors $\bm{B}_{f,i}^{l}=\left\{\bm{u}_{1,i}^{l}, \dots, \bm{u}_{k,i}^{l}\right\}$ from $\bm{U}_{f,i}^{l}$, capturing directions with the highest singular values. Similarly, the feature matrix $\bm{R}_{r,i}^{l}$ for remaining classes $\mathbf{D_{r,i}}$ defines the subspace $\mathcal{S}_{r,i}^{l} = \text{span} \left\{\bm{B}_{r,i}^{l}\right\}$. The two sets of layer-wised feature subspace, $\{\mathcal{S}_{f,i}^{1}, \dots,\mathcal{S}_{f,i}^{m}\}$ and $\{\mathcal{S}_{r,i}^{1}, \dots,\mathcal{S}_{r,i}^{m}\}$, represent the core part for forgetting and remaining classes, respectively, isolating features to be erased while preserving those to retain. By explicitly decomposing feature subspaces across all layers, we strengthen supervision signals for parameter updates and mitigate the risk of gradient obfuscation \cite{athalye2018obfuscated} in deep networks, where gradient inaccuracies caused by layer-wise nonlinear transformations could otherwise weaken the unlearning effect. This multi-layer alignment ensures consistent suppression of forgotten class features throughout the network hierarchy.



% 最后加一句我们在多个layer都做了这样的空间分解来加强对每层权重的监督信号这里可以引用carlini的gradient obfuscation的文章，说明层数很多的时候，梯度信息会不准确，所以我们要在多层都加这样的信号监督


% 这一段的符号可以想办法简化一下，比如：最开始不考虑是第几层layer，所有符号都没有上标L，然后最后加一句我们在多个layer都做了这样的空间分解来加强对每层权重的监督信号.这里可以引用carlini的gradient obfuscation的文章，说明层数很多的时候，梯度信息会不准确，所以我们要在多层都加这样的信号监督

% \cite{athalye2018obfuscated}




% according to the following criteria for the given threshold, $\epsilon$:
% \begin{align}
%     ||(\bm{R}_{f,i}^{l})_{k}||_{F}^{2} \geq \epsilon ||\bm{R}_{f,i}^{l}||_{F}^{2}.
% \end{align}
% We define the subspace, $\mathcal{S}_{f,i}^{l} = \text{span} \left\{\bm{B}_{f,i}^{l}\right\}$, where $\bm{B}_{f,i}^{l}=\left\{\bm{u}_{1,i}^{l}, \dots, \bm{u}_{k,i}^{l}\right\}$ consists of the first $k$ vectors in $\bm{U}_{f,i}^{l}$, as the space of significant representations for task $i$ at layer $l$. This subspace captures all directions corresponding to the highest singular values in the representation. Similarly, for each layer $l$, we construct the feature matrix $\bm{R}_{r,i}^{l}$ using only the forgetting data from task 1, $\mathbf{D_{r,i}}$, and obtain the corresponding subspace, $\mathcal{S}_{r,i}^{l}$. The sets $\{\mathcal{S}_{f,i}^{1}, \dots,\mathcal{S}_{f,i}^{m}\}$ and $\{\mathcal{S}_{r,i}^{1}, \dots,\mathcal{S}_{r,i}^{m}\}$ represent the disentangled feature spaces for the forgetting and remaining data, respectively. The former solely captures the features to be forgotten, while the latter preserves the features that should be retained.
% \subsection{Dual Orthogonal Projection}
% Model training involves two key processes: forward computation, which governs feature extraction, and backward propagation, which updates model parameters via gradient optimization. To achieve effective unlearning, it is essential to constrain both aspects to ensure that forgotten-class information is removed while retaining-class information remains intact. We propose an explicit **feature-level** and **gradient-level** constraint mechanism, implemented through a dual orthogonal projection framework.

% Before performing an unlearning task $\mathcal{T}_1$, we freeze both the backbone and classification head of the PTM \cite{zhao2025practical} and insert lightweight LoRA modules \cite{hu2022lora} at each layer. We denote the model with LoRA inserted as $\mathcal{M}_{\theta}$, where $\theta$ represents the trainable parameters in LoRA. After training, the learned updates $\theta^{*}$ are merged into the initial backbone weights, yielding $\mathcal{M}_{0} \overset{\theta^{*}}{\underset{\text{merge}}{\longrightarrow}} \mathcal{M}_{1}$.

% To enforce precise control over forgetting and retention, we propose a **dual orthogonal projection mechanism**, consisting of four key components: **Feature Orthogonal Projection for Forgetting (FOP-F)**, **Feature Orthogonal Projection for Retaining (FOP-R)**, **Gradient Orthogonal Projection for Forgetting (GOP-F)**, and **Gradient Orthogonal Projection for Retaining (GOP-R)**.

% \subsubsection{Feature Orthogonal Projection}
% To ensure effective unlearning at the feature level, we decompose the feature space into two subspaces: **the forgetting subspace $\mathcal{S}_{f,i}^{l}$**, which captures the discriminative features of the classes to be removed, and **the retaining subspace $\mathcal{S}_{r,i}^{l}$**, which encodes the features of the retained classes. The goal is to remove residual class-specific information for forgetting classes while ensuring the retained features remain aligned with their original representations.

% \textbf{FOP-F: Orthogonalizing Forgetting-Class Features.} For a batch of forgetting samples ${x_{f}}$ from $\mathbf{D_{f,i}}$, let $f_{l}({x_{f}})$ denote the feature vector at the $l$-th layer of the unlearned model $\mathcal{M}_{\theta}$. To achieve complete forgetting, $f_{l}({x_{f}})$ must be orthogonal to the feature subspace $\mathcal{S}_{f,i}^{l}$ spanned by the original model $\mathcal{M}$'s features. The optimal condition is:

% \begin{proposition}[FOP-F: Feature Orthogonal Projection for Forgetting]
% \label{proposition_1}
% Let ${x_{f}}$ denote a batch of forgetting samples from $\mathbf{D_{f,i}}$, and let $f_{l}({x_{f}})$ denote the feature vectors at the $l$-th layer of the unlearned model $\mathcal{M}_{\theta}$. For complete forgetting, $f_{l}({x_{f}})$ must deviate maximally from the feature subspace $\mathcal{S}_{f,i}^{l}$ spanned by the original model $\mathcal{M}$'s features. The optimal condition is absolute orthogonality: 
% \begin{align}
% f_l({x_f})^{\top} \mathcal{S}_{f,i}^l = \bm{0}.
% \end{align}
% \end{proposition}

% To enforce this globally, we minimize the nuclear norm of the projection:
% \begin{align}
% \mathcal{L}_{\text{FOP-F}} = \sum_{l=1}^{m} \|f_{l}({x_{f}})^{\top} \bm{B}_{f,i}^{l}\|_*,
% \end{align}
% where $\bm{B}_{f,i}^{l}$ represents the orthogonal bases for subspace $\mathcal{S}_{f,i}^{l}$. By driving the singular values in this term towards zero, we enforce orthogonality and eliminate residual class-specific information.

% \textbf{FOP-R: Aligning Retained-Class Features.} For a batch of remaining samples ${x_{r}}$ from $\mathbf{D_{r,i}}$, let $f_{l}({x_{r}})$ denote the corresponding feature vector. To preserve retained knowledge, we ensure that $f_{l}({x_{r}})$ aligns closely with the feature subspace $\mathcal{S}_{r,i}^{l}$ spanned by the original model's retained-class features. The optimal condition is minimizing the projection residual:

% \begin{proposition}[FOP-R: Feature Orthogonal Projection for Retaining]
% \label{proposition_2}
% Let ${x_{r}}$ denote a batch of remaining samples from $\mathbf{D_{r,i}}$, and let $f_{l}({x_{r}})$ denote the feature vectors at the $l$-th layer of the unlearned model $\mathcal{M}_{\theta}$. To preserve retained-class information, $f_{l}({x_{r}})$ must align closely with the feature subspace $\mathcal{S}_{r,i}^{l}$ spanned by the original model $\mathcal{M}$'s features. The optimal condition is minimal projection residual: 
% \begin{align}
% ||f_{l}({x_{r}}) - f_{l}({x_{r}})\mathbf{P}_{l}||_F^2 = 0.
% \end{align}
% \end{proposition}

% The corresponding loss function is:
% \begin{align}
% \mathcal{L}_{\text{FOP-R}} = \sum_{l=1}^{m} ||f_{l}({x_{r}}) - f_{l}({x_{r}})\mathbf{P}_{l}||_F^2,
% \end{align}
% where $\mathbf{P}_{l}=\mathbf{B}_{r,i}^{l}{(\mathbf{B}_{r,i}^{l})}^{\top}$ is the projection matrix for $\mathcal{S}_{r,i}^{l}$.

% \subsubsection{Gradient Orthogonal Projection}
% Beyond feature space constraints, we regulate gradient updates to prevent knowledge reactivation. Inspired by \cite{saha2021gradient}, which shows that gradients lie in the span of input features, we ensure that updates reinforce forgetting while preserving retained knowledge.

% \textbf{GOP-F: Forgetting-Class Gradient Projection.} Given the gradient $\bm{g_{l}}$ for parameters in layer $l$, computed via backpropagation, we first modify the gradient to ensure that updates occur only in the subspace $\mathcal{S}_{f,i}^{l}$:
% \begin{align}
% \bm{g'_{l}} = \bm{g_{l}}(\bm{I} - \mathbf{B}_{f,i}^{l}{(\mathbf{B}_{f,i}^{l})}^{\top}).
% \end{align}

% \textbf{GOP-R: Retained-Class Gradient Projection.} To prevent contamination of retained features, we further modify the gradient to remove components that interfere with the retaining subspace:
% \begin{align}
% \bm{g''_{l}} = \bm{g_{l}}\mathbf{B}_{r,i}^{l}{(\mathbf{B}_{r,i}^{l})}^{\top}.
% \end{align}

% The final gradient update is:
% \begin{align}
% \hat{\bm{g_{l}}} = \bm{g_{l}} - \bm{g'_{l}} - \bm{g''_{l}}.
% \end{align}

% \subsubsection{Final Optimization Objective}
% Combining both feature and gradient constraints, our final objective function is:
% \begin{align}
% \mathcal{L}_{\text{total}} = \mathcal{L}_{ce} + \lambda_1 \mathcal{L}_{\text{FOP-F}} + \lambda_2 \mathcal{L}_{\text{FOP-R}} + \lambda_3 \sum_{l=1}^{m} ||\bm{g'_{l}}||_F^2 + \lambda_4 \sum_{l=1}^{m} ||\bm{g''_{l}}||_F^2.
% \end{align}






\clearpage
\setcounter{page}{1}
\maketitlesupplementary


\setcounter{section}{0} % Reset section counter to 0
\setcounter{subsection}{0} % Reset subsection counter to 0
\setcounter{theorem}{0} % Reset subsection counter to 0
\setcounter{lemma}{0} % Reset subsection counter to 0



% \section{Proof}

% \subsection{Proof of 1}

% \begin{theorem}[Orthogonality of Subspaces]
% Let $S_1, S_2 \subset \mathbb{R}^n$ be $b$-dimensional subspaces spanned by orthonormal bases $B_1, B_2 \in \mathbb{R}^{n \times b}$ respectively, where $B_1^\top B_1 = I$ and $B_2^\top B_2 = I$. If all principal angles $\theta_i$ between $S_1$ and $S_2$ are $90^\circ$, then $S_1$ and $S_2$ are orthogonal (i.e., completely uncorrelated).
% \end{theorem}

% \begin{proof}
% \begin{enumerate}
%     \item \textbf{Principal angles and singular values}:\\
%     Define the matrix $M = B_1^\top B_2 \in \mathbb{R}^{b \times b}$. The singular values $\sigma_1 \geq \cdots \geq \sigma_b \geq 0$ of $M$ satisfy:
%     \[
%     \cos\theta_i = \sigma_i \quad \text{for all } i = 1,\ldots,b.
%     \]
    
%     \item \textbf{All angles at $90^\circ$}:\\
%     If $\theta_i = 90^\circ$ for all $i$, then $\cos\theta_i = 0$. Consequently, all singular values of $M$ vanish:
%     \[
%     \Sigma = \begin{bmatrix} 0 & \cdots & 0 \\ \vdots & \ddots & \vdots \\ 0 & \cdots & 0 \end{bmatrix} \implies M = U\Sigma V^\top = 0.
%     \]
    
%     \item \textbf{Orthogonality propagation}:\\
%     Since $M = B_1^\top B_2 = 0$, every basis vector in $B_1$ is orthogonal to every basis vector in $B_2$. For any $u \in S_1$ and $v \in S_2$, there exist coefficient vectors $\alpha, \beta \in \mathbb{R}^b$ such that:
%     \[
%     u = B_1\alpha, \quad v = B_2\beta \implies u^\top v = \alpha^\top (B_1^\top B_2)\beta = \alpha^\top 0\beta = 0.
%     \]
%     Thus, $S_1 \perp S_2$.
    
%     \item \textbf{Nuclear norm quantification}:\\
%     The nuclear norm $\|M\|_* = \sum_{i=1}^b \sigma_i = 0$ confirms complete orthogonality.
% \end{enumerate}
% \end{proof}


% \subsection{Proof of 2}

% \begin{theorem}[Identity of Subspaces]
% Under the same conditions, if all principal angles $\theta_i = 0^\circ$, then $S_1 = S_2$.
% \end{theorem}

% \begin{proof}
% \begin{enumerate}
%     \item \textbf{Singular values at maximum}:\\
%     If $\theta_i = 0^\circ$ for all $i$, then $\cos\theta_i = 1$. The singular values of $M$ become $\sigma_i = 1$, and the SVD reduces to:
%     \[
%     \Sigma = I \implies M = UI V^\top = UV^\top,
%     \]
%     where $UV^\top$ is an orthogonal matrix ($M^\top M = I$).
    
%     \item \textbf{Basis equivalence}:\\
%     From $M = B_1^\top B_2$ and the orthogonality of $M$, we derive:
%     \[
%     B_2 = B_1M.
%     \]
%     Since orthogonal transformations preserve spans, we have:
%     \[
%     \text{span}(B_2) = \text{span}(B_1M) = \text{span}(B_1) \implies S_1 = S_2.
%     \]
    
%     \item \textbf{Nuclear norm maximization}:\\
%     The nuclear norm reaches its maximum value $\|M\|_* = \sum_{i=1}^b 1 = b$, confirming subspace identity.
% \end{enumerate}
% \end{proof}




% \subsection{Proof of lemma1}

% % ========== Supporting Lemma ==========
% \begin{lemma}[Equivalence of Principal Angles and Singular Values]
% For any two subspaces $S_1, S_2$, the cosines of their principal angles equal the singular values of $M = B_1^\top B_2$.
% \end{lemma}

% \begin{proof}
% Through the Cosine-Sine (CS) decomposition, the matrix $M$ can be block-diagonalized as:
% \[
% M = \begin{bmatrix} \cos\Theta & -\sin\Theta \\ \sin\Theta & \cos\Theta \end{bmatrix},
% \]
% where $\cos\Theta$ contains $\cos\theta_i$ on its diagonal, corresponding to the singular values.
% \end{proof}









\begin{figure*}[t]
  \centering
   \includegraphics[width=1.0\linewidth]{appendix_fig/tsne_npy_20250303seed_42_1_tsne_visualization.pdf}
   \vspace{-4mm}
   \caption{{Accuracy on forgotten classes when recovering.} The \textcolor{blue}{line} (Pre-train) is the result before forgetting. The \textcolor{orange}{line} (Head Forgetting) is the trivial masking method. The \textcolor{red}{line} (Backbone Forgetting) is Our methods.}
   \label{fig:tsne}
   \vspace{-2mm}  
\end{figure*}




\begin{figure*}[t]
  \centering
   \includegraphics[width=1.0\linewidth]{appendix_fig/tsne_npy_20250303seed_42_3_tsne_visualization.pdf}
   \vspace{-4mm}
   \caption{{Accuracy on forgotten classes when recovering.} The \textcolor{blue}{line} (Pre-train) is the result before forgetting. The \textcolor{orange}{line} (Head Forgetting) is the trivial masking method. The \textcolor{red}{line} (Backbone Forgetting) is Our methods.}
   \label{fig:tsne}
   \vspace{-2mm}  
\end{figure*}


\begin{figure*}[t]
  \centering
   \includegraphics[width=1.0\linewidth]{appendix_fig/tsne_npy_20250303seed_42_4_tsne_visualization.pdf}
   \vspace{-4mm}
   \caption{{Accuracy on forgotten classes when recovering.} The \textcolor{blue}{line} (Pre-train) is the result before forgetting. The \textcolor{orange}{line} (Head Forgetting) is the trivial masking method. The \textcolor{red}{line} (Backbone Forgetting) is Our methods.}
   \label{fig:tsne}
   \vspace{-2mm}  
\end{figure*}



% \begin{figure*}[t]
%   \centering
%    \includegraphics[width=1.0\linewidth]{appendix_fig/tsne_npy_20250303seed_1337_1_tsne_visualization.pdf}
%    \vspace{-4mm}
%    \caption{{Accuracy on forgotten classes when recovering.} The \textcolor{blue}{line} (Pre-train) is the result before forgetting. The \textcolor{orange}{line} (Head Forgetting) is the trivial masking method. The \textcolor{red}{line} (Backbone Forgetting) is Our methods.}
%    \label{fig:tsne}
%    \vspace{-2mm}  
% \end{figure*}

% \begin{figure*}[t]
%   \centering
%    \includegraphics[width=1.0\linewidth]{appendix_fig/tsne_npy_20250303seed_1337_2_tsne_visualization.pdf}
%    \vspace{-4mm}
%    \caption{{Accuracy on forgotten classes when recovering.} The \textcolor{blue}{line} (Pre-train) is the result before forgetting. The \textcolor{orange}{line} (Head Forgetting) is the trivial masking method. The \textcolor{red}{line} (Backbone Forgetting) is Our methods.}
%    \label{fig:tsne}
%    \vspace{-2mm}  
% \end{figure*}

% \begin{figure*}[t]
%   \centering
%    \includegraphics[width=1.0\linewidth]{appendix_fig/tsne_npy_20250303seed_1337_3_tsne_visualization.pdf}
%    \vspace{-4mm}
%    \caption{{Accuracy on forgotten classes when recovering.} The \textcolor{blue}{line} (Pre-train) is the result before forgetting. The \textcolor{orange}{line} (Head Forgetting) is the trivial masking method. The \textcolor{red}{line} (Backbone Forgetting) is Our methods.}
%    \label{fig:tsne}
%    \vspace{-2mm}  
% \end{figure*}


% \begin{figure*}[t]
%   \centering
%    \includegraphics[width=1.0\linewidth]{appendix_fig/tsne_npy_20250303seed_1337_4_tsne_visualization.pdf}
%    \vspace{-4mm}
%    \caption{{Accuracy on forgotten classes when recovering.} The \textcolor{blue}{line} (Pre-train) is the result before forgetting. The \textcolor{orange}{line} (Head Forgetting) is the trivial masking method. The \textcolor{red}{line} (Backbone Forgetting) is Our methods.}
%    \label{fig:tsne}
%    \vspace{-2mm}  
% \end{figure*}






\begin{figure*}[!h]
    \centering
    \vspace{-2mm}
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./fig/ablated_lamda1_figure.pdf}
        \caption{Ablations on $\lambda_1$ condition with $\lambda_2=1$.}
        \label{fig:ablation_1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./fig/ablated_lamda2_figure.pdf}
        \caption{Ablations on $\lambda_2$ condition with $\lambda_1=0.2$.}
        \label{fig:ablation_2}
    \end{subfigure}
    \vspace{-4mm}
    \caption{Ablation studies on $\lambda_1$ and $\lambda_2$ on ImageNet100 of continual forgetting.}
    \label{fig:ablation_all}
    \vspace{-6mm}
\end{figure*}


\noindent
\textbf{Impact of Balancing Coefficients.}
\noindent
To elucidate the impact of coefficients in Eq.(\ref{eq:total_loss}) on the performance on both forgetting and remaining, we perform experiments on different $\lambda_{1}$ and $\lambda_{2}$ settings and the results are depicted in Figure \ref{fig:ablation_all}. We set the value of $\lambda_{1}$ as \{0.1, 0.2, 0.5, 1, 5\} successively, and find that the model can reach the optimal state when $\lambda_{1}$ = 1. Similarly, we vary the value of $\lambda_{2}$ as \{0.1, 0.2, 0.5, 1, 5\} successively, and observe that oure method achieves highest accuracy when $\lambda_{2}$ equals 0.2.





\section{appendix}

\noindent\textbf{Overview.} In this supplementary material, we submit the source code in the ``CE\_SDWV" folder and provide more experiments about our method. In Section~\ref{sec:Word Vocabulary and Sentence Generation Process}, we present a detailed process of constructing the word vocabulary and sentences. In Section~\ref{sec:Implementation Details}, we provide the specifics of our experiment setup. We then offer a deeper analysis of the parameter settings and present insightful findings in Section~\ref{sec:Additional Analysis}. More samples of our method are provided in Section~\ref{sec:More Samples} and preliminaries of diffusion models are presented in Section~\ref{sec:Preliminaries}. Finally, we discuss the societal impacts in Section~\ref{sec:Societal Impacts}.





1.实验细节
包括使用的数据集的介绍、benchmark的介绍，预训练模型的介绍（大小，结构）

2.超参数的选择

3.伪代码

4.更多的实验结果







4.1放三个实验结果conitnual forgetting，omni，cub，ms-sub100
\begin{table*}[t!]
\centering
\small
%\resizebox{\textwidth}{!}{%
% \setlength{\tabcolsep}{3.0pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllllllllllllll}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{3}{c}{\textit{Task 1}(100-20)} & \multicolumn{4}{c}{\textit{Task 2}(80-20)} & \multicolumn{4}{c}{\textit{Task 3}(60-20)} & \multicolumn{4}{c}{\textit{Task 4}(40-20)} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-8} \cmidrule(lr){9-12} \cmidrule(lr){13-16}
 & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $Acc_o \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $Acc_o \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $Acc_o \downarrow$ \\ \midrule
Pre-train & - & 74.31 & 74.65 & - & 74.50 & 73.80 & - & - & 74.80 & 73.91 & - & - & 74.47 & 75.11 & - \\
\midrule
% \multicolumn{5}{l}{\textcolor{orange}{\textit{(a) continual learning methods}}} \\
L2$^*$ & 66.91 & 62.13 & 2.16 & 66.66 & 61.74 & 1.37 & 9.36 & 66.42 & 61.37 & 1.54 & 11.83 & 66.95 & 61.02 & 0.97 &8.00 \\
EWC$^*$ \cite{kirkpatrick2017overcoming} &67.71  & 61.95 & {0.00} & 67.71 & 62.55 & {0.00} & \textbf{{0.00}} & 67.09 &61.43  &0.00  & {0.10} & 68.02 & 62.14 &0.00  &{0.23}  \\
MAS$^*$\cite{aljundi2018memory} & 67.52 & 61.63 & 0.00 & 68.12 & 63.25 & 0.00 & \textbf{{0.00}}& 68.15 & 63.23 &  {0.00}& \underline{0.03}   & 67.70 & 61.61 &{0.00} &\textbf{0.00} \\
LwF \cite{li2017learning}&69.43&65.04&0.21&69.94&66.47&0.00&0.21&70.34&67.11&0.00&\textbf{{0.00}}&70.89&67.12&0.00&\underline{0.04} \\
DER \cite{buzzega2020dark}&70.75&67.24&0.00&68.88&64.58&0.00&\textbf{{0.00}}&68.95&64.62&0.00&\textbf{{0.00}}&69.41&64.51&0.00&\textbf{0.00}\\
DER++ \cite{buzzega2020dark}&70.01&65.90&0.00&68.99&64.77&0.00&\textbf{{0.00}}&69.96&66.42&0.00&\textbf{{0.00}}&69.85&65.28&0.00&\textbf{0.00}\\
FDR \cite{benjamin2018measuring}&68.29&62.92&0.00&67.39&62.01&0.00&\textbf{{0.00}}&69.16&64.99&0.00&\textbf{{0.00}}&72.51&70.08&0.00&\textbf{0.00}\\
\midrule
% \multicolumn{5}{l}{\textcolor{orange}{\textit{(b) machine unlearning methods}}} \\
Retrain &17.29&9.77&{0.00}&31.12&19.72&{0.00}&\textbf{{0.00}}&41.17&28.80&{1.72}&\textbf{{0.00}}&52.44&41.77&4.66&{0.09} \\
BAD-T \cite{chundawat2023can}& 70.39 & 66.59 & {0.00} & 70.55 & 67.85 & {0.32} & \textbf{{0.00}} & 71.01 & 68.33 & {0.00} & {0.44} & 73.36 & 71.68 & 0.00 &{0.05} \\
LIRF$^*$ \cite{Ye2022LearningWR}& 30.59 & 64.46 & 54.60 & 34.05 & 62.03 & 50.34 & {43.50}& 44.56 & 62.53 &  {39.29}& {36.58}   & 40.36 & 62.62 &45.34 &27.96 \\
SCRUB  \cite{kurmanji2023towards}& 70.39 & 66.59 & {0.00} & 70.55 & 67.85 & {0.32} & \textbf{{0.00}} & 71.01 & 68.33 & {0.00} & {0.44} & 73.36 & 71.68 & 0.00 &{0.05} \\
SCRUB-S  \cite{kurmanji2023towards}&72.41  & 70.34 & {0.05} & {70.06}& {71.53} & {5.16} & {15.22} & {73.38}&73.09 &{0.24} & {15.81} & \underline{75.33} & 76.24 &{0.68}  &{6.47}  \\
% \rowcolor{yellow!50} % 另一行颜色
GS-LoRA \cite{zhao2024continual} & \underline{74.40} & {74.16} & 0.00 & \underline{73.59} & {73.37} &  0.00& \underline{0.05} & \underline{{74.36}} & {74.88} & 0.06 & \textbf{{0.00}} & {73.76} & {72.45} & 0.00 &{1.93} \\ 
% \rowcolor{yellow!50} %
GS-LoRA++ \cite{zhao2025practical} & {73.97} & {74.16} & 0.00 & {73.48} & {73.16} &  0.00& {0.10} & {74.20} & {74.51} & 0.00 & \textbf{{0.00} }& {75.23} & {75.36} & 0.00 &\textbf{0.00} \\
\midrule
\rowcolor{gray!30} % 设置当前行颜色
FEAST & \textbf{74.45} & {74.25} & 0.00 & \textbf{74.64} & {75.50} &  0.00 & \textbf{0.00} & \textbf{75.49} & {77.14} & 0.00 & \textbf{{0.00} }& \textbf{77.71} & {80.51} & 0.00 &\textbf{0.00} \\
\bottomrule
\end{tabular}%
}
%}
\caption{{Continual forgetting results for face recognition task on CASIA-Face100.} $Acc_o \ (\%)$ is the accuracy of old tasks, \ie, the accuracy on all previously forgotten classes in task $\mathcal{T}_1,\dots,\mathcal{T}_{t-1}$. There are 4 tasks in total and 20 classes are forgotten in each task. Considering desired forgetting should consider $Acc_r$ and $Acc_f$ at the same time, we only  \textbf{bold} and \underline{underline} the best and second best $H$ results respectively. }
\label{tab:cl-recog-caisa100}
\end{table*}


\begin{table*}[t!]
\centering
\small
%\resizebox{\textwidth}{!}{%
% \setlength{\tabcolsep}{3.0pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllllllllllllll}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{3}{c}{\textit{Task 1}(100-20)} & \multicolumn{4}{c}{\textit{Task 2}(80-20)} & \multicolumn{4}{c}{\textit{Task 3}(60-20)} & \multicolumn{4}{c}{\textit{Task 4}(40-20)} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-8} \cmidrule(lr){9-12} \cmidrule(lr){13-16}
 & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $Acc_o \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $Acc_o \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $Acc_o \downarrow$ \\ \midrule
Pre-train & - & 74.31 & 74.65 & - & 74.50 & 73.80 & - & - & 74.80 & 73.91 & - & - & 74.47 & 75.11 & - \\
\midrule
% \multicolumn{5}{l}{\textcolor{orange}{\textit{(a) continual learning methods}}} \\
L2$^*$ & 66.91 & 62.13 & 2.16 & 66.66 & 61.74 & 1.37 & 9.36 & 66.42 & 61.37 & 1.54 & 11.83 & 66.95 & 61.02 & 0.97 &8.00 \\
EWC$^*$ \cite{kirkpatrick2017overcoming} &67.71  & 61.95 & {0.00} & 67.71 & 62.55 & {0.00} & \textbf{{0.00}} & 67.09 &61.43  &0.00  & {0.10} & 68.02 & 62.14 &0.00  &{0.23}  \\
MAS$^*$\cite{aljundi2018memory} & 67.52 & 61.63 & 0.00 & 68.12 & 63.25 & 0.00 & \textbf{{0.00}}& 68.15 & 63.23 &  {0.00}& \underline{0.03}   & 67.70 & 61.61 &{0.00} &\textbf{0.00} \\
LwF \cite{li2017learning}&69.43&65.04&0.21&69.94&66.47&0.00&0.21&70.34&67.11&0.00&\textbf{{0.00}}&70.89&67.12&0.00&\underline{0.04} \\
DER \cite{buzzega2020dark}&70.75&67.24&0.00&68.88&64.58&0.00&\textbf{{0.00}}&68.95&64.62&0.00&\textbf{{0.00}}&69.41&64.51&0.00&\textbf{0.00}\\
DER++ \cite{buzzega2020dark}&70.01&65.90&0.00&68.99&64.77&0.00&\textbf{{0.00}}&69.96&66.42&0.00&\textbf{{0.00}}&69.85&65.28&0.00&\textbf{0.00}\\
FDR \cite{benjamin2018measuring}&68.29&62.92&0.00&67.39&62.01&0.00&\textbf{{0.00}}&69.16&64.99&0.00&\textbf{{0.00}}&72.51&70.08&0.00&\textbf{0.00}\\
\midrule
% \multicolumn{5}{l}{\textcolor{orange}{\textit{(b) machine unlearning methods}}} \\
Retrain &17.29&9.77&{0.00}&31.12&19.72&{0.00}&\textbf{{0.00}}&41.17&28.80&{1.72}&\textbf{{0.00}}&52.44&41.77&4.66&{0.09} \\
BAD-T \cite{chundawat2023can}& 70.39 & 66.59 & {0.00} & 70.55 & 67.85 & {0.32} & \textbf{{0.00}} & 71.01 & 68.33 & {0.00} & {0.44} & 73.36 & 71.68 & 0.00 &{0.05} \\
LIRF$^*$ \cite{Ye2022LearningWR}& 30.59 & 64.46 & 54.60 & 34.05 & 62.03 & 50.34 & {43.50}& 44.56 & 62.53 &  {39.29}& {36.58}   & 40.36 & 62.62 &45.34 &27.96 \\
SCRUB  \cite{kurmanji2023towards}& 70.39 & 66.59 & {0.00} & 70.55 & 67.85 & {0.32} & \textbf{{0.00}} & 71.01 & 68.33 & {0.00} & {0.44} & 73.36 & 71.68 & 0.00 &{0.05} \\
SCRUB-S  \cite{kurmanji2023towards}&72.41  & 70.34 & {0.05} & {70.06}& {71.53} & {5.16} & {15.22} & {73.38}&73.09 &{0.24} & {15.81} & \underline{75.33} & 76.24 &{0.68}  &{6.47}  \\
% \rowcolor{yellow!50} % 另一行颜色
GS-LoRA \cite{zhao2024continual} & \underline{74.40} & {74.16} & 0.00 & \underline{73.59} & {73.37} &  0.00& \underline{0.05} & \underline{{74.36}} & {74.88} & 0.06 & \textbf{{0.00}} & {73.76} & {72.45} & 0.00 &{1.93} \\ 
% \rowcolor{yellow!50} %
GS-LoRA++ \cite{zhao2025practical} & {73.97} & {74.16} & 0.00 & {73.48} & {73.16} &  0.00& {0.10} & {74.20} & {74.51} & 0.00 & \textbf{{0.00} }& {75.23} & {75.36} & 0.00 &\textbf{0.00} \\
\midrule
\rowcolor{gray!30} % 设置当前行颜色
FEAST & \textbf{74.45} & {74.25} & 0.00 & \textbf{74.64} & {75.50} &  0.00 & \textbf{0.00} & \textbf{75.49} & {77.14} & 0.00 & \textbf{{0.00} }& \textbf{77.71} & {80.51} & 0.00 &\textbf{0.00} \\
\bottomrule
\end{tabular}%
}
%}
\caption{{Continual forgetting results for face recognition task on CASIA-Face100.} $Acc_o \ (\%)$ is the accuracy of old tasks, \ie, the accuracy on all previously forgotten classes in task $\mathcal{T}_1,\dots,\mathcal{T}_{t-1}$. There are 4 tasks in total and 20 classes are forgotten in each task. Considering desired forgetting should consider $Acc_r$ and $Acc_f$ at the same time, we only  \textbf{bold} and \underline{underline} the best and second best $H$ results respectively. }
\label{tab:cl-recog-caisa100}
\end{table*}


\begin{table*}[t!]
\centering
\small
%\resizebox{\textwidth}{!}{%
% \setlength{\tabcolsep}{3.0pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllllllllllllll}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{3}{c}{\textit{Task 1}(100-20)} & \multicolumn{4}{c}{\textit{Task 2}(80-20)} & \multicolumn{4}{c}{\textit{Task 3}(60-20)} & \multicolumn{4}{c}{\textit{Task 4}(40-20)} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-8} \cmidrule(lr){9-12} \cmidrule(lr){13-16}
 & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $Acc_o \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $Acc_o \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $Acc_o \downarrow$ \\ \midrule
Pre-train & - & 74.31 & 74.65 & - & 74.50 & 73.80 & - & - & 74.80 & 73.91 & - & - & 74.47 & 75.11 & - \\
\midrule
% \multicolumn{5}{l}{\textcolor{orange}{\textit{(a) continual learning methods}}} \\
L2$^*$ & 66.91 & 62.13 & 2.16 & 66.66 & 61.74 & 1.37 & 9.36 & 66.42 & 61.37 & 1.54 & 11.83 & 66.95 & 61.02 & 0.97 &8.00 \\
EWC$^*$ \cite{kirkpatrick2017overcoming} &67.71  & 61.95 & {0.00} & 67.71 & 62.55 & {0.00} & \textbf{{0.00}} & 67.09 &61.43  &0.00  & {0.10} & 68.02 & 62.14 &0.00  &{0.23}  \\
MAS$^*$\cite{aljundi2018memory} & 67.52 & 61.63 & 0.00 & 68.12 & 63.25 & 0.00 & \textbf{{0.00}}& 68.15 & 63.23 &  {0.00}& \underline{0.03}   & 67.70 & 61.61 &{0.00} &\textbf{0.00} \\
LwF \cite{li2017learning}&69.43&65.04&0.21&69.94&66.47&0.00&0.21&70.34&67.11&0.00&\textbf{{0.00}}&70.89&67.12&0.00&\underline{0.04} \\
DER \cite{buzzega2020dark}&70.75&67.24&0.00&68.88&64.58&0.00&\textbf{{0.00}}&68.95&64.62&0.00&\textbf{{0.00}}&69.41&64.51&0.00&\textbf{0.00}\\
DER++ \cite{buzzega2020dark}&70.01&65.90&0.00&68.99&64.77&0.00&\textbf{{0.00}}&69.96&66.42&0.00&\textbf{{0.00}}&69.85&65.28&0.00&\textbf{0.00}\\
FDR \cite{benjamin2018measuring}&68.29&62.92&0.00&67.39&62.01&0.00&\textbf{{0.00}}&69.16&64.99&0.00&\textbf{{0.00}}&72.51&70.08&0.00&\textbf{0.00}\\
\midrule
% \multicolumn{5}{l}{\textcolor{orange}{\textit{(b) machine unlearning methods}}} \\
Retrain &17.29&9.77&{0.00}&31.12&19.72&{0.00}&\textbf{{0.00}}&41.17&28.80&{1.72}&\textbf{{0.00}}&52.44&41.77&4.66&{0.09} \\
BAD-T \cite{chundawat2023can}& 70.39 & 66.59 & {0.00} & 70.55 & 67.85 & {0.32} & \textbf{{0.00}} & 71.01 & 68.33 & {0.00} & {0.44} & 73.36 & 71.68 & 0.00 &{0.05} \\
LIRF$^*$ \cite{Ye2022LearningWR}& 30.59 & 64.46 & 54.60 & 34.05 & 62.03 & 50.34 & {43.50}& 44.56 & 62.53 &  {39.29}& {36.58}   & 40.36 & 62.62 &45.34 &27.96 \\
SCRUB  \cite{kurmanji2023towards}& 70.39 & 66.59 & {0.00} & 70.55 & 67.85 & {0.32} & \textbf{{0.00}} & 71.01 & 68.33 & {0.00} & {0.44} & 73.36 & 71.68 & 0.00 &{0.05} \\
SCRUB-S  \cite{kurmanji2023towards}&72.41  & 70.34 & {0.05} & {70.06}& {71.53} & {5.16} & {15.22} & {73.38}&73.09 &{0.24} & {15.81} & \underline{75.33} & 76.24 &{0.68}  &{6.47}  \\
% \rowcolor{yellow!50} % 另一行颜色
GS-LoRA \cite{zhao2024continual} & \underline{74.40} & {74.16} & 0.00 & \underline{73.59} & {73.37} &  0.00& \underline{0.05} & \underline{{74.36}} & {74.88} & 0.06 & \textbf{{0.00}} & {73.76} & {72.45} & 0.00 &{1.93} \\ 
% \rowcolor{yellow!50} %
GS-LoRA++ \cite{zhao2025practical} & {73.97} & {74.16} & 0.00 & {73.48} & {73.16} &  0.00& {0.10} & {74.20} & {74.51} & 0.00 & \textbf{{0.00} }& {75.23} & {75.36} & 0.00 &\textbf{0.00} \\
\midrule
\rowcolor{gray!30} % 设置当前行颜色
FEAST & \textbf{74.45} & {74.25} & 0.00 & \textbf{74.64} & {75.50} &  0.00 & \textbf{0.00} & \textbf{75.49} & {77.14} & 0.00 & \textbf{{0.00} }& \textbf{77.71} & {80.51} & 0.00 &\textbf{0.00} \\
\bottomrule
\end{tabular}%
}
%}
\caption{{Continual forgetting results for face recognition task on CASIA-Face100.} $Acc_o \ (\%)$ is the accuracy of old tasks, \ie, the accuracy on all previously forgotten classes in task $\mathcal{T}_1,\dots,\mathcal{T}_{t-1}$. There are 4 tasks in total and 20 classes are forgotten in each task. Considering desired forgetting should consider $Acc_r$ and $Acc_f$ at the same time, we only  \textbf{bold} and \underline{underline} the best and second best $H$ results respectively. }
\label{tab:cl-recog-caisa100}
\end{table*}
关于the main results


% \setlength{\tabcolsep}{1.0mm}{
\begin{table}[t!]
  \centering
    % \vspace{-2mm}
    \small
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{lll|lll}
  \toprule
    % \multirow{2}{*}{Ablated Variants} & \multicolumn{2}{c}{\textcolor{orange}{\textit{Task 1}}} & \multicolumn{3}{c}{\textcolor{orange}{\textit{Task 2}}} \\
    \multirow{2}{*}{Variants} & \multirow{2}{*}{Construct} & \multirow{2}{*}{Constraint} & \multicolumn{3}{c}{{\textit{Task 2(80-20)}}} \\
    \cmidrule(lr){4-6} 
    & & & $Acc_r$ $\uparrow$ & $Acc_f$ $\downarrow$ & $Acc_o$ $\downarrow$ \\
    \midrule 
    Pre-train  & - & - & 90.03 & 89.60 & - \\
    \rowcolor{gray!30} % 设置当前行颜色
    % FEAST  & 86.73 & 0.10 & 87.43 & 0.10 & 0.10 \\
    \textit{Variant1} & class token & class token & 87.43 & 0.10 & 0.10 \\
    \textit{Variant2} & class token & all tokens & 90.67 & 51.10 & 38.80 \\
    \textit{Variant3} & all tokens & class token & 84.30 & 0.3 & 0.10 \\
    \textit{Variant4} & all tokens & all tokens & 86.78 & 0.12 & 0.28 \\
    % \quad w/\textit{atten.} & 73.92 & 0.10 & 76.58 & 4.37 & 0.82 \\  
    % \quad w/\textit{pool.} & 73.92 & 0.05 & 74.98 & 0.21 & 0.15 \\
     % && \gr{+1.72} & - & \bluegr{-0.49} & \bluegr{-8} \\
  \bottomrule
\end{tabular}
}
\vspace{-2mm}
\caption{Different implementations for construction of the feature subspace and the constraint during forward. Here, \textit{Variant1} is the default setting in FEAST.}
\label{tab:subspace}
\vspace{-5mm}
\end{table}
% }



4.2不同数量的single-step遗忘
machine unlearning

这里要放五个benchmark上的结果，imagenet100，casia100，omni，cub，ms-sub100

只放我们自己的结果即可




\begin{table*}[t!]
\centering
\vspace{-5pt}
% \renewcommand{\arraystretch}{1.1}
% \setlength{\tabcolsep}{6pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrr}
\toprule
\multirow{2}{*}{Methods} &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Tunable\\ Ratio $\downarrow$ \end{tabular}} & \multicolumn{3}{c}{100-5} & \multicolumn{3}{c}{100-10} & \multicolumn{3}{c}{100-50} & \multicolumn{3}{c}{100-90} \\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14} 
 && $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ \\ \midrule
Pre-train & - & - & 73.85 &  70.88& -  & 73.81 & 72.74 & - & 72.45 & 74.88 & - & 72.32 & 73.86 \\
\midrule
% \multicolumn{5}{l}{\textcolor{orange}{\textit{(a) continual learning methods}}} \\
L2$^*$& 99.73\% & 67.13 & 66.96 & 3.58 & 67.74& 64.87&1.86& 64.39 & 56.61 & 0.24 & 52.45 & 40.68 & 0.04  \\
GS-LoRA \cite{zhao2024continual} &\textbf{1.28\%}& {71.02} & {71.16} & 0.00 & {71.76} & {70.81} & {0.00}  & {71.29} & {68.05} & 0.02 & {73.71} & {73.56} & 0.00 \\
GS-LoRA++ \cite{zhao2025practical} &\textbf{1.28\%}& {71.12} & {71.36} & 0.00 & {72.04} & {71.35} & {0.00}  & {71.56} & {68.52} & 0.00 & {72.85} & {71.86} & 0.00 \\ 
\midrule
\rowcolor{gray!30} % 设置当前行颜色
FEAST &\textbf{1.28\%}& \textbf{71.78} & {72.71} & {0.00} & \textbf{72.52} & {72.31} & {0.00}  & \textbf{74.18} & {73.51} & {0.00} & \textbf{75.49} & {77.15} & {0.00} \\ 
\bottomrule
\end{tabular}%
}
\caption{{Single-step forgetting results for face recognition task on CASIA-Face100.} $Acc_r\ (\%)$ and $Acc_f\ (\%)$ are the accuracies of remaining and forgotten classes.
$^*$~denotes the original methods with a rehearsal buffer.
Retrain represents retraining the model using replay data and \textit{the training epoch is the same as other methods to ensure a fair comparison.} Pre-train denotes the results before forgetting.
All setting is in the form of 100-Y, which means all experiments start from a pre-trained model (100 classes originally) and forget Y classes.}
\label{tab:single-recog-caisa100}
\vspace{-0pt}
\end{table*}




\begin{table*}[t!]
\centering
\vspace{-5pt}
% \renewcommand{\arraystretch}{1.1}
% \setlength{\tabcolsep}{6pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrr}
\toprule
\multirow{2}{*}{Methods} &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Tunable\\ Ratio $\downarrow$ \end{tabular}} & \multicolumn{3}{c}{100-5} & \multicolumn{3}{c}{100-10} & \multicolumn{3}{c}{100-50} & \multicolumn{3}{c}{100-90} \\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14} 
 && $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ \\ \midrule
Pre-train & - & - & 73.85 &  70.88& -  & 73.81 & 72.74 & - & 72.45 & 74.88 & - & 72.32 & 73.86 \\
\midrule
% \multicolumn{5}{l}{\textcolor{orange}{\textit{(a) continual learning methods}}} \\
L2$^*$& 99.73\% & 67.13 & 66.96 & 3.58 & 67.74& 64.87&1.86& 64.39 & 56.61 & 0.24 & 52.45 & 40.68 & 0.04  \\
GS-LoRA \cite{zhao2024continual} &\textbf{1.28\%}& {71.02} & {71.16} & 0.00 & {71.76} & {70.81} & {0.00}  & {71.29} & {68.05} & 0.02 & {73.71} & {73.56} & 0.00 \\
GS-LoRA++ \cite{zhao2025practical} &\textbf{1.28\%}& {71.12} & {71.36} & 0.00 & {72.04} & {71.35} & {0.00}  & {71.56} & {68.52} & 0.00 & {72.85} & {71.86} & 0.00 \\ 
\midrule
\rowcolor{gray!30} % 设置当前行颜色
FEAST &\textbf{1.28\%}& \textbf{71.78} & {72.71} & {0.00} & \textbf{72.52} & {72.31} & {0.00}  & \textbf{74.18} & {73.51} & {0.00} & \textbf{75.49} & {77.15} & {0.00} \\ 
\bottomrule
\end{tabular}%
}
\caption{{Single-step forgetting results for face recognition task on CASIA-Face100.} $Acc_r\ (\%)$ and $Acc_f\ (\%)$ are the accuracies of remaining and forgotten classes.
$^*$~denotes the original methods with a rehearsal buffer.
Retrain represents retraining the model using replay data and \textit{the training epoch is the same as other methods to ensure a fair comparison.} Pre-train denotes the results before forgetting.
All setting is in the form of 100-Y, which means all experiments start from a pre-trained model (100 classes originally) and forget Y classes.}
\label{tab:single-recog-caisa100}
\vspace{-0pt}
\end{table*}



\begin{table*}[t!]
\centering
\vspace{-5pt}
% \renewcommand{\arraystretch}{1.1}
% \setlength{\tabcolsep}{6pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrr}
\toprule
\multirow{2}{*}{Methods} &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Tunable\\ Ratio $\downarrow$ \end{tabular}} & \multicolumn{3}{c}{100-5} & \multicolumn{3}{c}{100-10} & \multicolumn{3}{c}{100-50} & \multicolumn{3}{c}{100-90} \\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14} 
 && $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ \\ \midrule
Pre-train & - & - & 73.85 &  70.88& -  & 73.81 & 72.74 & - & 72.45 & 74.88 & - & 72.32 & 73.86 \\
\midrule
% \multicolumn{5}{l}{\textcolor{orange}{\textit{(a) continual learning methods}}} \\
L2$^*$& 99.73\% & 67.13 & 66.96 & 3.58 & 67.74& 64.87&1.86& 64.39 & 56.61 & 0.24 & 52.45 & 40.68 & 0.04  \\
GS-LoRA \cite{zhao2024continual} &\textbf{1.28\%}& {71.02} & {71.16} & 0.00 & {71.76} & {70.81} & {0.00}  & {71.29} & {68.05} & 0.02 & {73.71} & {73.56} & 0.00 \\
GS-LoRA++ \cite{zhao2025practical} &\textbf{1.28\%}& {71.12} & {71.36} & 0.00 & {72.04} & {71.35} & {0.00}  & {71.56} & {68.52} & 0.00 & {72.85} & {71.86} & 0.00 \\ 
\midrule
\rowcolor{gray!30} % 设置当前行颜色
FEAST &\textbf{1.28\%}& \textbf{71.78} & {72.71} & {0.00} & \textbf{72.52} & {72.31} & {0.00}  & \textbf{74.18} & {73.51} & {0.00} & \textbf{75.49} & {77.15} & {0.00} \\ 
\bottomrule
\end{tabular}%
}
\caption{{Single-step forgetting results for face recognition task on CASIA-Face100.} $Acc_r\ (\%)$ and $Acc_f\ (\%)$ are the accuracies of remaining and forgotten classes.
$^*$~denotes the original methods with a rehearsal buffer.
Retrain represents retraining the model using replay data and \textit{the training epoch is the same as other methods to ensure a fair comparison.} Pre-train denotes the results before forgetting.
All setting is in the form of 100-Y, which means all experiments start from a pre-trained model (100 classes originally) and forget Y classes.}
\label{tab:single-recog-caisa100}
\vspace{-0pt}
\end{table*}



\begin{table*}[t!]
\centering
\vspace{-5pt}
% \renewcommand{\arraystretch}{1.1}
% \setlength{\tabcolsep}{6pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrr}
\toprule
\multirow{2}{*}{Methods} &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Tunable\\ Ratio $\downarrow$ \end{tabular}} & \multicolumn{3}{c}{100-5} & \multicolumn{3}{c}{100-10} & \multicolumn{3}{c}{100-50} & \multicolumn{3}{c}{100-90} \\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14} 
 && $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ \\ \midrule
Pre-train & - & - & 73.85 &  70.88& -  & 73.81 & 72.74 & - & 72.45 & 74.88 & - & 72.32 & 73.86 \\
\midrule
% \multicolumn{5}{l}{\textcolor{orange}{\textit{(a) continual learning methods}}} \\
L2$^*$& 99.73\% & 67.13 & 66.96 & 3.58 & 67.74& 64.87&1.86& 64.39 & 56.61 & 0.24 & 52.45 & 40.68 & 0.04  \\
GS-LoRA \cite{zhao2024continual} &\textbf{1.28\%}& {71.02} & {71.16} & 0.00 & {71.76} & {70.81} & {0.00}  & {71.29} & {68.05} & 0.02 & {73.71} & {73.56} & 0.00 \\
GS-LoRA++ \cite{zhao2025practical} &\textbf{1.28\%}& {71.12} & {71.36} & 0.00 & {72.04} & {71.35} & {0.00}  & {71.56} & {68.52} & 0.00 & {72.85} & {71.86} & 0.00 \\ 
\midrule
\rowcolor{gray!30} % 设置当前行颜色
FEAST &\textbf{1.28\%}& \textbf{71.78} & {72.71} & {0.00} & \textbf{72.52} & {72.31} & {0.00}  & \textbf{74.18} & {73.51} & {0.00} & \textbf{75.49} & {77.15} & {0.00} \\ 
\bottomrule
\end{tabular}%
}
\caption{{Single-step forgetting results for face recognition task on CASIA-Face100.} $Acc_r\ (\%)$ and $Acc_f\ (\%)$ are the accuracies of remaining and forgotten classes.
$^*$~denotes the original methods with a rehearsal buffer.
Retrain represents retraining the model using replay data and \textit{the training epoch is the same as other methods to ensure a fair comparison.} Pre-train denotes the results before forgetting.
All setting is in the form of 100-Y, which means all experiments start from a pre-trained model (100 classes originally) and forget Y classes.}
\label{tab:single-recog-caisa100}
\vspace{-0pt}
\end{table*}



\begin{table*}[t!]
\centering
\vspace{-5pt}
% \renewcommand{\arraystretch}{1.1}
% \setlength{\tabcolsep}{6pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrr}
\toprule
\multirow{2}{*}{Methods} &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Tunable\\ Ratio $\downarrow$ \end{tabular}} & \multicolumn{3}{c}{100-5} & \multicolumn{3}{c}{100-10} & \multicolumn{3}{c}{100-50} & \multicolumn{3}{c}{100-90} \\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14} 
 && $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ \\ \midrule
Pre-train & - & - & 73.85 &  70.88& -  & 73.81 & 72.74 & - & 72.45 & 74.88 & - & 72.32 & 73.86 \\
\midrule
% \multicolumn{5}{l}{\textcolor{orange}{\textit{(a) continual learning methods}}} \\
L2$^*$& 99.73\% & 67.13 & 66.96 & 3.58 & 67.74& 64.87&1.86& 64.39 & 56.61 & 0.24 & 52.45 & 40.68 & 0.04  \\
GS-LoRA \cite{zhao2024continual} &\textbf{1.28\%}& {71.02} & {71.16} & 0.00 & {71.76} & {70.81} & {0.00}  & {71.29} & {68.05} & 0.02 & {73.71} & {73.56} & 0.00 \\
GS-LoRA++ \cite{zhao2025practical} &\textbf{1.28\%}& {71.12} & {71.36} & 0.00 & {72.04} & {71.35} & {0.00}  & {71.56} & {68.52} & 0.00 & {72.85} & {71.86} & 0.00 \\ 
\midrule
\rowcolor{gray!30} % 设置当前行颜色
FEAST &\textbf{1.28\%}& \textbf{71.78} & {72.71} & {0.00} & \textbf{72.52} & {72.31} & {0.00}  & \textbf{74.18} & {73.51} & {0.00} & \textbf{75.49} & {77.15} & {0.00} \\ 
\bottomrule
\end{tabular}%
}
\caption{{Single-step forgetting results for face recognition task on CASIA-Face100.} $Acc_r\ (\%)$ and $Acc_f\ (\%)$ are the accuracies of remaining and forgotten classes.
$^*$~denotes the original methods with a rehearsal buffer.
Retrain represents retraining the model using replay data and \textit{the training epoch is the same as other methods to ensure a fair comparison.} Pre-train denotes the results before forgetting.
All setting is in the form of 100-Y, which means all experiments start from a pre-trained model (100 classes originally) and forget Y classes.}
\label{tab:single-recog-caisa100}
\vspace{-0pt}
\end{table*}



\begin{algorithm}[t]
\caption{Pseudo code of CE-SDWV}\label{alg:CE-SDWV}
\begin{algorithmic}
\STATE \textbf{Input:} diffusion model $F_\theta(\cdot)$, input text condition $p$, text encoder $\Gamma(\cdot)$, diffusion steps $T$, target concept $\mathcal{X}_t$, optimization timestep $t_\theta \in [0,T]$, sampling step $t = 0$, learning rate $\eta$
\STATE \textbf{Stage One:}
\STATE Collect augmentation sentences $\{s_i\}_{i=0}^{N}$ and corresponding token indices $id_{i,j}$ related to target concept $\mathcal{X}_t$
\STATE $\bm{R}_t \gets$ CONCAT($\Gamma(s_i)[id_{i,j}]$)
\STATE ${\bm{U}_t}{\bm\Sigma}_t{\bm{V}_t^T} \gets \text{SVD}(\bm{R}_t)$
\STATE $\bm{\hat R}_t \gets \bm{U}_t[:k]\bm\Sigma_t[:k]\bm{V}_t^T[:k]$
\STATE $\bm{B}_t \gets \bm{U}_t[:k]$
\STATE \textbf{Stage Two:}
\STATE $\bm{\hat c} \gets \Gamma(p)$
\FOR{each $\bm{\hat c}_i$ in $\bm{\hat c}$}
    \STATE $\bm{\hat R}_t^{\prime} \gets$ CONCAT($\bm{\hat c}_i,\bm{\hat R}_t$)
    \STATE ${\bm{U}_t^{\prime}}\bm{\Sigma}_t^{\prime}{\bm{V}_t^{\prime T}} \gets \text{SVD}(\bm{\hat R}_t^{\prime})$
    \STATE $\bm{\Sigma}_t^{\prime}[:k] \gets 0$
    \STATE $\bm{\hat c}_i^{\prime} \gets ({\bm{U}_t^{\prime}}\bm{\Sigma}_t^{\prime}{\bm{V}_t^{\prime T}})[0]$ 
\ENDFOR
\STATE $\bm{\hat c}^{\prime} \gets \{\bm{\hat c}_i^{\prime}\}_{i=0}^{n}$
\STATE \textbf{Stage Three:}
\FOR{each $t$ in RANGE($t_\theta,T$)}
    \STATE $\bm{\epsilon}_{t-1}^{*} \gets F_\theta(\bm{x}_t, t, \bm{\hat c})$
    \STATE $\bm{\epsilon}_{t-1} \gets F_\theta(\bm{x}_t, t, \bm{\hat c}^{\prime})$
    \STATE $\mathcal{L}_{\text{noise-guide}} \gets \left\|\bm{\hat\epsilon}_{t} - \bm{\epsilon}_{t}\right\|^{2}$
    \STATE $\bm{g}_{\bm{\hat c}^{\prime}} \gets \nabla_{\bm{\hat c}^{\prime}}\mathcal{L}_{\text{noise-guide}}$
    \STATE $\bm{g}_{\bm{\hat c}^{\prime}}^{\bot} \gets {\bm{g}_{\bm{\hat c}^{\prime}}}{\bm{B}_t}\left({\bm{B}_t}\right)^{T}$
    \STATE $\bm{\hat c}^{\prime} \gets \bm{\hat c}^{\prime} - \eta\bm{g}_{\bm{\hat c}^{\prime}}^{\bot}$
    \STATE $\bm{x}_{t-1} \gets \text{STEP}(\bm{x}_t, \bm{\epsilon}_{t-1}, t)$
\ENDFOR
\end{algorithmic}
\end{algorithm}




4.--1.disentangled feature subspace的构建和相应的disturb-denoise的实现方式
Table \ref{tab:subspace}

4.-.lora加在不同的地方，attention or ffn

4.1subspace构建的时候需要 $\epsilon$这个参数对于性能的影响，消融

4.3核范数的设计有什么优势？

讲核范数能够在趋向于正交的同时尽可能使得低秩，因此在forgetting上更有好处，但是在remaining上只需要和补空间正交不需要其他的约束，因此L2 norm已经够了。
给实验结果


4.2continual forgetting on 更多的数据集上和benchmark上

4.3single-step forgetting 
1-99，体现的是我们方法的可扩展性


3.遗忘的恢复效果
在imageNet100上的恢复效果

4.更多的tsne图


face上的图
4.1.forget5remain10得图还有7x3张，
7行3列

4.2.大图100类得1张
图太大了，可能需要放到三个页面

4.3要不要加imageNet100的图？？


5.更多的实验结果关于特征还原

5.1提供还原的方法，ae
5.2还原的过程，iteration 
5.3还原的不同层的特征以及对应的psnr和ssim
5.4对于forgetting data和remaining data都进行这一步。要强调的是
对于forgetting data的还原，我们比他们差；对于remaining data的还原，我们比他们好，更加接近于原始特征










% % 进 task with 4 task 20 classes unlearning classes



% % , MS-Celeb-100, and OmniBenchmark 的IU



% % 以下三个角度对our methods进行验证: (1) 更大的模型，where we adopt the 



% % 在更广泛的数据集, \ie, CUB-200, MS-Celeb-100, and OmniBenchmark进行了更
 


% % compared the results of model adaptation with 




% % different incremental stages to determine the best solution in model adaptation. We also explore the influence of hyper-parameters in model adaptation, \eg, the prompt length in VPT and the projection dimension in Adapter. Additionally, we provide additional Grad-CAM results for better visualization.





% % \noindent Following \cite{zhao2024continual}, we evaluate FG-OrIU on classification and face recognition tasks. For classification, we use ImageNet100 \cite{russakovsky2015imagenet}, CUB-200 \cite{wah2011caltech}, and Omnibenchmark \cite{zhang2022benchmarking}, with a ViT-B/16 \cite{dosovitskiy2020image} pre-trained in PyTorch \cite{paszke2019pytorch}. For face recognition, we use CASIA-Face100 \cite{zhao2024continual}, a subset of CASIA-WebFace \cite{yi2014learning}, and MS-Celeb-100, sampled from \cite{guo2016ms}. The pre-trained model is the Face Transformer from \cite{zhong2021face}. We focus on class-unlearning scenarios: in MU, varying numbers of classes are removed; in IU, 20 classes are removed per task over 4 tasks. More details are in Appendix.


% \begin{figure*}[t]
%   \centering
%    \includegraphics[width=1.0\linewidth]{appendix_fig/tsne_npy_20250303seed_42_1_tsne_visualization.pdf}
%    \vspace{-4mm}
%    \caption{{Accuracy on forgotten classes when recovering.} The \textcolor{blue}{line} (Pre-train) is the result before forgetting. The \textcolor{orange}{line} (Head Forgetting) is the trivial masking method. The \textcolor{red}{line} (Backbone Forgetting) is Our methods.}
%    \label{fig:tsne}
%    \vspace{-2mm}  
% \end{figure*}

% \begin{figure*}[t]
%   \centering
%    \includegraphics[width=1.0\linewidth]{appendix_fig/tsne_npy_20250303seed_42_3_tsne_visualization.pdf}
%    \vspace{-4mm}
%    \caption{{Accuracy on forgotten classes when recovering.} The \textcolor{blue}{line} (Pre-train) is the result before forgetting. The \textcolor{orange}{line} (Head Forgetting) is the trivial masking method. The \textcolor{red}{line} (Backbone Forgetting) is Our methods.}
%    \label{fig:tsne}
%    \vspace{-2mm}  
% \end{figure*}

% \begin{figure*}[t]
%   \centering
%    \includegraphics[width=1.0\linewidth]{appendix_fig/tsne_npy_20250303seed_42_4_tsne_visualization.pdf}
%    \vspace{-4mm}
%    \caption{{Accuracy on forgotten classes when recovering.} The \textcolor{blue}{line} (Pre-train) is the result before forgetting. The \textcolor{orange}{line} (Head Forgetting) is the trivial masking method. The \textcolor{red}{line} (Backbone Forgetting) is Our methods.}
%    \label{fig:tsne}
%    \vspace{-2mm}  
% \end{figure*}



% % \begin{figure*}[t]
% %   \centering
% %    \includegraphics[width=1.0\linewidth]{appendix_fig/tsne_npy_20250303seed_1337_1_tsne_visualization.pdf}
% %    \vspace{-4mm}
% %    \caption{{Accuracy on forgotten classes when recovering.} The \textcolor{blue}{line} (Pre-train) is the result before forgetting. The \textcolor{orange}{line} (Head Forgetting) is the trivial masking method. The \textcolor{red}{line} (Backbone Forgetting) is Our methods.}
% %    \label{fig:tsne}
% %    \vspace{-2mm}  
% % \end{figure*}

% % \begin{figure*}[t]
% %   \centering
% %    \includegraphics[width=1.0\linewidth]{appendix_fig/tsne_npy_20250303seed_1337_2_tsne_visualization.pdf}
% %    \vspace{-4mm}
% %    \caption{{Accuracy on forgotten classes when recovering.} The \textcolor{blue}{line} (Pre-train) is the result before forgetting. The \textcolor{orange}{line} (Head Forgetting) is the trivial masking method. The \textcolor{red}{line} (Backbone Forgetting) is Our methods.}
% %    \label{fig:tsne}
% %    \vspace{-2mm}  
% % \end{figure*}

% % \begin{figure*}[t]
% %   \centering
% %    \includegraphics[width=1.0\linewidth]{appendix_fig/tsne_npy_20250303seed_1337_3_tsne_visualization.pdf}
% %    \vspace{-4mm}
% %    \caption{{Accuracy on forgotten classes when recovering.} The \textcolor{blue}{line} (Pre-train) is the result before forgetting. The \textcolor{orange}{line} (Head Forgetting) is the trivial masking method. The \textcolor{red}{line} (Backbone Forgetting) is Our methods.}
% %    \label{fig:tsne}
% %    \vspace{-2mm}  
% % \end{figure*}


% % \begin{figure*}[t]
% %   \centering
% %    \includegraphics[width=1.0\linewidth]{appendix_fig/tsne_npy_20250303seed_1337_4_tsne_visualization.pdf}
% %    \vspace{-4mm}
% %    \caption{{Accuracy on forgotten classes when recovering.} The \textcolor{blue}{line} (Pre-train) is the result before forgetting. The \textcolor{orange}{line} (Head Forgetting) is the trivial masking method. The \textcolor{red}{line} (Backbone Forgetting) is Our methods.}
% %    \label{fig:tsne}
% %    \vspace{-2mm}  
% % \end{figure*}






% \begin{figure*}[!h]
%     \centering
%     \vspace{-2mm}
%     \begin{subfigure}{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{./fig/ablated_lamda1_figure.pdf}
%         \caption{Ablations on $\lambda_1$ condition with $\lambda_2=1$.}
%         \label{fig:ablation_1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{./fig/ablated_lamda2_figure.pdf}
%         \caption{Ablations on $\lambda_2$ condition with $\lambda_1=0.2$.}
%         \label{fig:ablation_2}
%     \end{subfigure}
%     \vspace{-4mm}
%     \caption{Ablation studies on $\lambda_1$ and $\lambda_2$ on ImageNet100 of continual forgetting.}
%     \label{fig:ablation_all}
%     \vspace{-6mm}
% \end{figure*}












% % 1.实验细节
% % 包括使用的数据集的介绍、benchmark的介绍，预训练模型的介绍（大小，结构）

% % 2.超参数的选择

% % 3.伪代码

% % 4.更多的实验结果







% % 4.1放三个实验结果conitnual forgetting，omni，cub，ms-sub100
% \begin{table*}[t!]
% \centering
% \small
% %\resizebox{\textwidth}{!}{%
% % \setlength{\tabcolsep}{3.0pt}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llllllllllllllll}
% \toprule
% \multirow{2}{*}{Methods} & \multicolumn{3}{c}{\textit{Task 1}(100-20)} & \multicolumn{4}{c}{\textit{Task 2}(80-20)} & \multicolumn{4}{c}{\textit{Task 3}(60-20)} & \multicolumn{4}{c}{\textit{Task 4}(40-20)} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-8} \cmidrule(lr){9-12} \cmidrule(lr){13-16}
%  & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $Acc_o \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $Acc_o \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $Acc_o \downarrow$ \\ \midrule
% Pre-train & - & 74.31 & 74.65 & - & 74.50 & 73.80 & - & - & 74.80 & 73.91 & - & - & 74.47 & 75.11 & - \\
% \midrule
% % \multicolumn{5}{l}{\textcolor{orange}{\textit{(a) continual learning methods}}} \\
% L2$^*$ & 66.91 & 62.13 & 2.16 & 66.66 & 61.74 & 1.37 & 9.36 & 66.42 & 61.37 & 1.54 & 11.83 & 66.95 & 61.02 & 0.97 &8.00 \\
% EWC$^*$ \cite{kirkpatrick2017overcoming} &67.71  & 61.95 & {0.00} & 67.71 & 62.55 & {0.00} & \textbf{{0.00}} & 67.09 &61.43  &0.00  & {0.10} & 68.02 & 62.14 &0.00  &{0.23}  \\
% MAS$^*$\cite{aljundi2018memory} & 67.52 & 61.63 & 0.00 & 68.12 & 63.25 & 0.00 & \textbf{{0.00}}& 68.15 & 63.23 &  {0.00}& \underline{0.03}   & 67.70 & 61.61 &{0.00} &\textbf{0.00} \\
% LwF \cite{li2017learning}&69.43&65.04&0.21&69.94&66.47&0.00&0.21&70.34&67.11&0.00&\textbf{{0.00}}&70.89&67.12&0.00&\underline{0.04} \\
% DER \cite{buzzega2020dark}&70.75&67.24&0.00&68.88&64.58&0.00&\textbf{{0.00}}&68.95&64.62&0.00&\textbf{{0.00}}&69.41&64.51&0.00&\textbf{0.00}\\
% DER++ \cite{buzzega2020dark}&70.01&65.90&0.00&68.99&64.77&0.00&\textbf{{0.00}}&69.96&66.42&0.00&\textbf{{0.00}}&69.85&65.28&0.00&\textbf{0.00}\\
% FDR \cite{benjamin2018measuring}&68.29&62.92&0.00&67.39&62.01&0.00&\textbf{{0.00}}&69.16&64.99&0.00&\textbf{{0.00}}&72.51&70.08&0.00&\textbf{0.00}\\
% \midrule
% % \multicolumn{5}{l}{\textcolor{orange}{\textit{(b) machine unlearning methods}}} \\
% Retrain &17.29&9.77&{0.00}&31.12&19.72&{0.00}&\textbf{{0.00}}&41.17&28.80&{1.72}&\textbf{{0.00}}&52.44&41.77&4.66&{0.09} \\
% BAD-T \cite{chundawat2023can}& 70.39 & 66.59 & {0.00} & 70.55 & 67.85 & {0.32} & \textbf{{0.00}} & 71.01 & 68.33 & {0.00} & {0.44} & 73.36 & 71.68 & 0.00 &{0.05} \\
% LIRF$^*$ \cite{Ye2022LearningWR}& 30.59 & 64.46 & 54.60 & 34.05 & 62.03 & 50.34 & {43.50}& 44.56 & 62.53 &  {39.29}& {36.58}   & 40.36 & 62.62 &45.34 &27.96 \\
% SCRUB  \cite{kurmanji2023towards}& 70.39 & 66.59 & {0.00} & 70.55 & 67.85 & {0.32} & \textbf{{0.00}} & 71.01 & 68.33 & {0.00} & {0.44} & 73.36 & 71.68 & 0.00 &{0.05} \\
% SCRUB-S  \cite{kurmanji2023towards}&72.41  & 70.34 & {0.05} & {70.06}& {71.53} & {5.16} & {15.22} & {73.38}&73.09 &{0.24} & {15.81} & \underline{75.33} & 76.24 &{0.68}  &{6.47}  \\
% % \rowcolor{yellow!50} % 另一行颜色
% GS-LoRA \cite{zhao2024continual} & \underline{74.40} & {74.16} & 0.00 & \underline{73.59} & {73.37} &  0.00& \underline{0.05} & \underline{{74.36}} & {74.88} & 0.06 & \textbf{{0.00}} & {73.76} & {72.45} & 0.00 &{1.93} \\ 
% % \rowcolor{yellow!50} %
% GS-LoRA++ \cite{zhao2025practical} & {73.97} & {74.16} & 0.00 & {73.48} & {73.16} &  0.00& {0.10} & {74.20} & {74.51} & 0.00 & \textbf{{0.00} }& {75.23} & {75.36} & 0.00 &\textbf{0.00} \\
% \midrule
% \rowcolor{gray!30} % 设置当前行颜色
% FEAST & \textbf{74.45} & {74.25} & 0.00 & \textbf{74.64} & {75.50} &  0.00 & \textbf{0.00} & \textbf{75.49} & {77.14} & 0.00 & \textbf{{0.00} }& \textbf{77.71} & {80.51} & 0.00 &\textbf{0.00} \\
% \bottomrule
% \end{tabular}%
% }
% %}
% \caption{{Continual forgetting results for face recognition task on CASIA-Face100.} $Acc_o \ (\%)$ is the accuracy of old tasks, \ie, the accuracy on all previously forgotten classes in task $\mathcal{T}_1,\dots,\mathcal{T}_{t-1}$. There are 4 tasks in total and 20 classes are forgotten in each task. Considering desired forgetting should consider $Acc_r$ and $Acc_f$ at the same time, we only  \textbf{bold} and \underline{underline} the best and second best $H$ results respectively. }
% \label{tab:cl-recog-caisa100}
% \end{table*}


% \begin{table*}[t!]
% \centering
% \small
% %\resizebox{\textwidth}{!}{%
% % \setlength{\tabcolsep}{3.0pt}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llllllllllllllll}
% \toprule
% \multirow{2}{*}{Methods} & \multicolumn{3}{c}{\textit{Task 1}(100-20)} & \multicolumn{4}{c}{\textit{Task 2}(80-20)} & \multicolumn{4}{c}{\textit{Task 3}(60-20)} & \multicolumn{4}{c}{\textit{Task 4}(40-20)} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-8} \cmidrule(lr){9-12} \cmidrule(lr){13-16}
%  & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $Acc_o \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $Acc_o \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $Acc_o \downarrow$ \\ \midrule
% Pre-train & - & 74.31 & 74.65 & - & 74.50 & 73.80 & - & - & 74.80 & 73.91 & - & - & 74.47 & 75.11 & - \\
% \midrule
% % \multicolumn{5}{l}{\textcolor{orange}{\textit{(a) continual learning methods}}} \\
% L2$^*$ & 66.91 & 62.13 & 2.16 & 66.66 & 61.74 & 1.37 & 9.36 & 66.42 & 61.37 & 1.54 & 11.83 & 66.95 & 61.02 & 0.97 &8.00 \\
% EWC$^*$ \cite{kirkpatrick2017overcoming} &67.71  & 61.95 & {0.00} & 67.71 & 62.55 & {0.00} & \textbf{{0.00}} & 67.09 &61.43  &0.00  & {0.10} & 68.02 & 62.14 &0.00  &{0.23}  \\
% MAS$^*$\cite{aljundi2018memory} & 67.52 & 61.63 & 0.00 & 68.12 & 63.25 & 0.00 & \textbf{{0.00}}& 68.15 & 63.23 &  {0.00}& \underline{0.03}   & 67.70 & 61.61 &{0.00} &\textbf{0.00} \\
% LwF \cite{li2017learning}&69.43&65.04&0.21&69.94&66.47&0.00&0.21&70.34&67.11&0.00&\textbf{{0.00}}&70.89&67.12&0.00&\underline{0.04} \\
% DER \cite{buzzega2020dark}&70.75&67.24&0.00&68.88&64.58&0.00&\textbf{{0.00}}&68.95&64.62&0.00&\textbf{{0.00}}&69.41&64.51&0.00&\textbf{0.00}\\
% DER++ \cite{buzzega2020dark}&70.01&65.90&0.00&68.99&64.77&0.00&\textbf{{0.00}}&69.96&66.42&0.00&\textbf{{0.00}}&69.85&65.28&0.00&\textbf{0.00}\\
% FDR \cite{benjamin2018measuring}&68.29&62.92&0.00&67.39&62.01&0.00&\textbf{{0.00}}&69.16&64.99&0.00&\textbf{{0.00}}&72.51&70.08&0.00&\textbf{0.00}\\
% \midrule
% % \multicolumn{5}{l}{\textcolor{orange}{\textit{(b) machine unlearning methods}}} \\
% Retrain &17.29&9.77&{0.00}&31.12&19.72&{0.00}&\textbf{{0.00}}&41.17&28.80&{1.72}&\textbf{{0.00}}&52.44&41.77&4.66&{0.09} \\
% BAD-T \cite{chundawat2023can}& 70.39 & 66.59 & {0.00} & 70.55 & 67.85 & {0.32} & \textbf{{0.00}} & 71.01 & 68.33 & {0.00} & {0.44} & 73.36 & 71.68 & 0.00 &{0.05} \\
% LIRF$^*$ \cite{Ye2022LearningWR}& 30.59 & 64.46 & 54.60 & 34.05 & 62.03 & 50.34 & {43.50}& 44.56 & 62.53 &  {39.29}& {36.58}   & 40.36 & 62.62 &45.34 &27.96 \\
% SCRUB  \cite{kurmanji2023towards}& 70.39 & 66.59 & {0.00} & 70.55 & 67.85 & {0.32} & \textbf{{0.00}} & 71.01 & 68.33 & {0.00} & {0.44} & 73.36 & 71.68 & 0.00 &{0.05} \\
% SCRUB-S  \cite{kurmanji2023towards}&72.41  & 70.34 & {0.05} & {70.06}& {71.53} & {5.16} & {15.22} & {73.38}&73.09 &{0.24} & {15.81} & \underline{75.33} & 76.24 &{0.68}  &{6.47}  \\
% % \rowcolor{yellow!50} % 另一行颜色
% GS-LoRA \cite{zhao2024continual} & \underline{74.40} & {74.16} & 0.00 & \underline{73.59} & {73.37} &  0.00& \underline{0.05} & \underline{{74.36}} & {74.88} & 0.06 & \textbf{{0.00}} & {73.76} & {72.45} & 0.00 &{1.93} \\ 
% % \rowcolor{yellow!50} %
% GS-LoRA++ \cite{zhao2025practical} & {73.97} & {74.16} & 0.00 & {73.48} & {73.16} &  0.00& {0.10} & {74.20} & {74.51} & 0.00 & \textbf{{0.00} }& {75.23} & {75.36} & 0.00 &\textbf{0.00} \\
% \midrule
% \rowcolor{gray!30} % 设置当前行颜色
% FEAST & \textbf{74.45} & {74.25} & 0.00 & \textbf{74.64} & {75.50} &  0.00 & \textbf{0.00} & \textbf{75.49} & {77.14} & 0.00 & \textbf{{0.00} }& \textbf{77.71} & {80.51} & 0.00 &\textbf{0.00} \\
% \bottomrule
% \end{tabular}%
% }
% %}
% \caption{{Continual forgetting results for face recognition task on CASIA-Face100.} $Acc_o \ (\%)$ is the accuracy of old tasks, \ie, the accuracy on all previously forgotten classes in task $\mathcal{T}_1,\dots,\mathcal{T}_{t-1}$. There are 4 tasks in total and 20 classes are forgotten in each task. Considering desired forgetting should consider $Acc_r$ and $Acc_f$ at the same time, we only  \textbf{bold} and \underline{underline} the best and second best $H$ results respectively. }
% \label{tab:cl-recog-caisa100}
% \end{table*}


% \begin{table*}[t!]
% \centering
% \small
% %\resizebox{\textwidth}{!}{%
% % \setlength{\tabcolsep}{3.0pt}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llllllllllllllll}
% \toprule
% \multirow{2}{*}{Methods} & \multicolumn{3}{c}{\textit{Task 1}(100-20)} & \multicolumn{4}{c}{\textit{Task 2}(80-20)} & \multicolumn{4}{c}{\textit{Task 3}(60-20)} & \multicolumn{4}{c}{\textit{Task 4}(40-20)} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-8} \cmidrule(lr){9-12} \cmidrule(lr){13-16}
%  & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $Acc_o \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $Acc_o \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $Acc_o \downarrow$ \\ \midrule
% Pre-train & - & 74.31 & 74.65 & - & 74.50 & 73.80 & - & - & 74.80 & 73.91 & - & - & 74.47 & 75.11 & - \\
% \midrule
% % \multicolumn{5}{l}{\textcolor{orange}{\textit{(a) continual learning methods}}} \\
% L2$^*$ & 66.91 & 62.13 & 2.16 & 66.66 & 61.74 & 1.37 & 9.36 & 66.42 & 61.37 & 1.54 & 11.83 & 66.95 & 61.02 & 0.97 &8.00 \\
% EWC$^*$ \cite{kirkpatrick2017overcoming} &67.71  & 61.95 & {0.00} & 67.71 & 62.55 & {0.00} & \textbf{{0.00}} & 67.09 &61.43  &0.00  & {0.10} & 68.02 & 62.14 &0.00  &{0.23}  \\
% MAS$^*$\cite{aljundi2018memory} & 67.52 & 61.63 & 0.00 & 68.12 & 63.25 & 0.00 & \textbf{{0.00}}& 68.15 & 63.23 &  {0.00}& \underline{0.03}   & 67.70 & 61.61 &{0.00} &\textbf{0.00} \\
% LwF \cite{li2017learning}&69.43&65.04&0.21&69.94&66.47&0.00&0.21&70.34&67.11&0.00&\textbf{{0.00}}&70.89&67.12&0.00&\underline{0.04} \\
% DER \cite{buzzega2020dark}&70.75&67.24&0.00&68.88&64.58&0.00&\textbf{{0.00}}&68.95&64.62&0.00&\textbf{{0.00}}&69.41&64.51&0.00&\textbf{0.00}\\
% DER++ \cite{buzzega2020dark}&70.01&65.90&0.00&68.99&64.77&0.00&\textbf{{0.00}}&69.96&66.42&0.00&\textbf{{0.00}}&69.85&65.28&0.00&\textbf{0.00}\\
% FDR \cite{benjamin2018measuring}&68.29&62.92&0.00&67.39&62.01&0.00&\textbf{{0.00}}&69.16&64.99&0.00&\textbf{{0.00}}&72.51&70.08&0.00&\textbf{0.00}\\
% \midrule
% % \multicolumn{5}{l}{\textcolor{orange}{\textit{(b) machine unlearning methods}}} \\
% Retrain &17.29&9.77&{0.00}&31.12&19.72&{0.00}&\textbf{{0.00}}&41.17&28.80&{1.72}&\textbf{{0.00}}&52.44&41.77&4.66&{0.09} \\
% BAD-T \cite{chundawat2023can}& 70.39 & 66.59 & {0.00} & 70.55 & 67.85 & {0.32} & \textbf{{0.00}} & 71.01 & 68.33 & {0.00} & {0.44} & 73.36 & 71.68 & 0.00 &{0.05} \\
% LIRF$^*$ \cite{Ye2022LearningWR}& 30.59 & 64.46 & 54.60 & 34.05 & 62.03 & 50.34 & {43.50}& 44.56 & 62.53 &  {39.29}& {36.58}   & 40.36 & 62.62 &45.34 &27.96 \\
% SCRUB  \cite{kurmanji2023towards}& 70.39 & 66.59 & {0.00} & 70.55 & 67.85 & {0.32} & \textbf{{0.00}} & 71.01 & 68.33 & {0.00} & {0.44} & 73.36 & 71.68 & 0.00 &{0.05} \\
% SCRUB-S  \cite{kurmanji2023towards}&72.41  & 70.34 & {0.05} & {70.06}& {71.53} & {5.16} & {15.22} & {73.38}&73.09 &{0.24} & {15.81} & \underline{75.33} & 76.24 &{0.68}  &{6.47}  \\
% % \rowcolor{yellow!50} % 另一行颜色
% GS-LoRA \cite{zhao2024continual} & \underline{74.40} & {74.16} & 0.00 & \underline{73.59} & {73.37} &  0.00& \underline{0.05} & \underline{{74.36}} & {74.88} & 0.06 & \textbf{{0.00}} & {73.76} & {72.45} & 0.00 &{1.93} \\ 
% % \rowcolor{yellow!50} %
% GS-LoRA++ \cite{zhao2025practical} & {73.97} & {74.16} & 0.00 & {73.48} & {73.16} &  0.00& {0.10} & {74.20} & {74.51} & 0.00 & \textbf{{0.00} }& {75.23} & {75.36} & 0.00 &\textbf{0.00} \\
% \midrule
% \rowcolor{gray!30} % 设置当前行颜色
% FEAST & \textbf{74.45} & {74.25} & 0.00 & \textbf{74.64} & {75.50} &  0.00 & \textbf{0.00} & \textbf{75.49} & {77.14} & 0.00 & \textbf{{0.00} }& \textbf{77.71} & {80.51} & 0.00 &\textbf{0.00} \\
% \bottomrule
% \end{tabular}%
% }
% %}
% \caption{{Continual forgetting results for face recognition task on CASIA-Face100.} $Acc_o \ (\%)$ is the accuracy of old tasks, \ie, the accuracy on all previously forgotten classes in task $\mathcal{T}_1,\dots,\mathcal{T}_{t-1}$. There are 4 tasks in total and 20 classes are forgotten in each task. Considering desired forgetting should consider $Acc_r$ and $Acc_f$ at the same time, we only  \textbf{bold} and \underline{underline} the best and second best $H$ results respectively. }
% \label{tab:cl-recog-caisa100}
% \end{table*}
% % 关于the main results


% % \setlength{\tabcolsep}{1.0mm}{
% \begin{table}[t!]
%   \centering
%     % \vspace{-2mm}
%     \small
%   \resizebox{\columnwidth}{!}{
%   \begin{tabular}{lll|lll}
%   \toprule
%     % \multirow{2}{*}{Ablated Variants} & \multicolumn{2}{c}{\textcolor{orange}{\textit{Task 1}}} & \multicolumn{3}{c}{\textcolor{orange}{\textit{Task 2}}} \\
%     \multirow{2}{*}{Variants} & \multirow{2}{*}{Construct} & \multirow{2}{*}{Constraint} & \multicolumn{3}{c}{{\textit{Task 2(80-20)}}} \\
%     \cmidrule(lr){4-6} 
%     & & & $Acc_r$ $\uparrow$ & $Acc_f$ $\downarrow$ & $Acc_o$ $\downarrow$ \\
%     \midrule 
%     Pre-train  & - & - & 90.03 & 89.60 & - \\
%     \rowcolor{gray!30} % 设置当前行颜色
%     % FEAST  & 86.73 & 0.10 & 87.43 & 0.10 & 0.10 \\
%     \textit{Variant1} & class token & class token & 87.43 & 0.10 & 0.10 \\
%     \textit{Variant2} & class token & all tokens & 90.67 & 51.10 & 38.80 \\
%     \textit{Variant3} & all tokens & class token & 84.30 & 0.3 & 0.10 \\
%     \textit{Variant4} & all tokens & all tokens & 86.78 & 0.12 & 0.28 \\
%     % \quad w/\textit{atten.} & 73.92 & 0.10 & 76.58 & 4.37 & 0.82 \\  
%     % \quad w/\textit{pool.} & 73.92 & 0.05 & 74.98 & 0.21 & 0.15 \\
%      % && \gr{+1.72} & - & \bluegr{-0.49} & \bluegr{-8} \\
%   \bottomrule
% \end{tabular}
% }
% \vspace{-2mm}
% \caption{Different implementations for construction of the feature subspace and the constraint during forward. Here, \textit{Variant1} is the default setting in FEAST.}
% \label{tab:subspace}
% \vspace{-5mm}
% \end{table}
% % }



% % 4.2不同数量的single-step遗忘
% % machine unlearning

% % 这里要放五个benchmark上的结果，imagenet100，casia100，omni，cub，ms-sub100

% % 只放我们自己的结果即可




% \begin{table*}[t!]
% \centering
% \vspace{-5pt}
% % \renewcommand{\arraystretch}{1.1}
% % \setlength{\tabcolsep}{6pt}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lrrrrrrrrrrrrrr}
% \toprule
% \multirow{2}{*}{Methods} &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Tunable\\ Ratio $\downarrow$ \end{tabular}} & \multicolumn{3}{c}{100-5} & \multicolumn{3}{c}{100-10} & \multicolumn{3}{c}{100-50} & \multicolumn{3}{c}{100-90} \\ 
% \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14} 
%  && $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ \\ \midrule
% Pre-train & - & - & 73.85 &  70.88& -  & 73.81 & 72.74 & - & 72.45 & 74.88 & - & 72.32 & 73.86 \\
% \midrule
% % \multicolumn{5}{l}{\textcolor{orange}{\textit{(a) continual learning methods}}} \\
% L2$^*$& 99.73\% & 67.13 & 66.96 & 3.58 & 67.74& 64.87&1.86& 64.39 & 56.61 & 0.24 & 52.45 & 40.68 & 0.04  \\
% GS-LoRA \cite{zhao2024continual} &\textbf{1.28\%}& {71.02} & {71.16} & 0.00 & {71.76} & {70.81} & {0.00}  & {71.29} & {68.05} & 0.02 & {73.71} & {73.56} & 0.00 \\
% GS-LoRA++ \cite{zhao2025practical} &\textbf{1.28\%}& {71.12} & {71.36} & 0.00 & {72.04} & {71.35} & {0.00}  & {71.56} & {68.52} & 0.00 & {72.85} & {71.86} & 0.00 \\ 
% \midrule
% \rowcolor{gray!30} % 设置当前行颜色
% FEAST &\textbf{1.28\%}& \textbf{71.78} & {72.71} & {0.00} & \textbf{72.52} & {72.31} & {0.00}  & \textbf{74.18} & {73.51} & {0.00} & \textbf{75.49} & {77.15} & {0.00} \\ 
% \bottomrule
% \end{tabular}%
% }
% \caption{{Single-step forgetting results for face recognition task on CASIA-Face100.} $Acc_r\ (\%)$ and $Acc_f\ (\%)$ are the accuracies of remaining and forgotten classes.
% $^*$~denotes the original methods with a rehearsal buffer.
% Retrain represents retraining the model using replay data and \textit{the training epoch is the same as other methods to ensure a fair comparison.} Pre-train denotes the results before forgetting.
% All setting is in the form of 100-Y, which means all experiments start from a pre-trained model (100 classes originally) and forget Y classes.}
% \label{tab:single-recog-caisa100}
% \vspace{-0pt}
% \end{table*}




% \begin{table*}[t!]
% \centering
% \vspace{-5pt}
% % \renewcommand{\arraystretch}{1.1}
% % \setlength{\tabcolsep}{6pt}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lrrrrrrrrrrrrrr}
% \toprule
% \multirow{2}{*}{Methods} &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Tunable\\ Ratio $\downarrow$ \end{tabular}} & \multicolumn{3}{c}{100-5} & \multicolumn{3}{c}{100-10} & \multicolumn{3}{c}{100-50} & \multicolumn{3}{c}{100-90} \\ 
% \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14} 
%  && $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ \\ \midrule
% Pre-train & - & - & 73.85 &  70.88& -  & 73.81 & 72.74 & - & 72.45 & 74.88 & - & 72.32 & 73.86 \\
% \midrule
% % \multicolumn{5}{l}{\textcolor{orange}{\textit{(a) continual learning methods}}} \\
% L2$^*$& 99.73\% & 67.13 & 66.96 & 3.58 & 67.74& 64.87&1.86& 64.39 & 56.61 & 0.24 & 52.45 & 40.68 & 0.04  \\
% GS-LoRA \cite{zhao2024continual} &\textbf{1.28\%}& {71.02} & {71.16} & 0.00 & {71.76} & {70.81} & {0.00}  & {71.29} & {68.05} & 0.02 & {73.71} & {73.56} & 0.00 \\
% GS-LoRA++ \cite{zhao2025practical} &\textbf{1.28\%}& {71.12} & {71.36} & 0.00 & {72.04} & {71.35} & {0.00}  & {71.56} & {68.52} & 0.00 & {72.85} & {71.86} & 0.00 \\ 
% \midrule
% \rowcolor{gray!30} % 设置当前行颜色
% FEAST &\textbf{1.28\%}& \textbf{71.78} & {72.71} & {0.00} & \textbf{72.52} & {72.31} & {0.00}  & \textbf{74.18} & {73.51} & {0.00} & \textbf{75.49} & {77.15} & {0.00} \\ 
% \bottomrule
% \end{tabular}%
% }
% \caption{{Single-step forgetting results for face recognition task on CASIA-Face100.} $Acc_r\ (\%)$ and $Acc_f\ (\%)$ are the accuracies of remaining and forgotten classes.
% $^*$~denotes the original methods with a rehearsal buffer.
% Retrain represents retraining the model using replay data and \textit{the training epoch is the same as other methods to ensure a fair comparison.} Pre-train denotes the results before forgetting.
% All setting is in the form of 100-Y, which means all experiments start from a pre-trained model (100 classes originally) and forget Y classes.}
% \label{tab:single-recog-caisa100}
% \vspace{-0pt}
% \end{table*}



% \begin{table*}[t!]
% \centering
% \vspace{-5pt}
% % \renewcommand{\arraystretch}{1.1}
% % \setlength{\tabcolsep}{6pt}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lrrrrrrrrrrrrrr}
% \toprule
% \multirow{2}{*}{Methods} &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Tunable\\ Ratio $\downarrow$ \end{tabular}} & \multicolumn{3}{c}{100-5} & \multicolumn{3}{c}{100-10} & \multicolumn{3}{c}{100-50} & \multicolumn{3}{c}{100-90} \\ 
% \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14} 
%  && $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ \\ \midrule
% Pre-train & - & - & 73.85 &  70.88& -  & 73.81 & 72.74 & - & 72.45 & 74.88 & - & 72.32 & 73.86 \\
% \midrule
% % \multicolumn{5}{l}{\textcolor{orange}{\textit{(a) continual learning methods}}} \\
% L2$^*$& 99.73\% & 67.13 & 66.96 & 3.58 & 67.74& 64.87&1.86& 64.39 & 56.61 & 0.24 & 52.45 & 40.68 & 0.04  \\
% GS-LoRA \cite{zhao2024continual} &\textbf{1.28\%}& {71.02} & {71.16} & 0.00 & {71.76} & {70.81} & {0.00}  & {71.29} & {68.05} & 0.02 & {73.71} & {73.56} & 0.00 \\
% GS-LoRA++ \cite{zhao2025practical} &\textbf{1.28\%}& {71.12} & {71.36} & 0.00 & {72.04} & {71.35} & {0.00}  & {71.56} & {68.52} & 0.00 & {72.85} & {71.86} & 0.00 \\ 
% \midrule
% \rowcolor{gray!30} % 设置当前行颜色
% FEAST &\textbf{1.28\%}& \textbf{71.78} & {72.71} & {0.00} & \textbf{72.52} & {72.31} & {0.00}  & \textbf{74.18} & {73.51} & {0.00} & \textbf{75.49} & {77.15} & {0.00} \\ 
% \bottomrule
% \end{tabular}%
% }
% \caption{{Single-step forgetting results for face recognition task on CASIA-Face100.} $Acc_r\ (\%)$ and $Acc_f\ (\%)$ are the accuracies of remaining and forgotten classes.
% $^*$~denotes the original methods with a rehearsal buffer.
% Retrain represents retraining the model using replay data and \textit{the training epoch is the same as other methods to ensure a fair comparison.} Pre-train denotes the results before forgetting.
% All setting is in the form of 100-Y, which means all experiments start from a pre-trained model (100 classes originally) and forget Y classes.}
% \label{tab:single-recog-caisa100}
% \vspace{-0pt}
% \end{table*}



% \begin{table*}[t!]
% \centering
% \vspace{-5pt}
% % \renewcommand{\arraystretch}{1.1}
% % \setlength{\tabcolsep}{6pt}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lrrrrrrrrrrrrrr}
% \toprule
% \multirow{2}{*}{Methods} &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Tunable\\ Ratio $\downarrow$ \end{tabular}} & \multicolumn{3}{c}{100-5} & \multicolumn{3}{c}{100-10} & \multicolumn{3}{c}{100-50} & \multicolumn{3}{c}{100-90} \\ 
% \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14} 
%  && $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ \\ \midrule
% Pre-train & - & - & 73.85 &  70.88& -  & 73.81 & 72.74 & - & 72.45 & 74.88 & - & 72.32 & 73.86 \\
% \midrule
% % \multicolumn{5}{l}{\textcolor{orange}{\textit{(a) continual learning methods}}} \\
% L2$^*$& 99.73\% & 67.13 & 66.96 & 3.58 & 67.74& 64.87&1.86& 64.39 & 56.61 & 0.24 & 52.45 & 40.68 & 0.04  \\
% GS-LoRA \cite{zhao2024continual} &\textbf{1.28\%}& {71.02} & {71.16} & 0.00 & {71.76} & {70.81} & {0.00}  & {71.29} & {68.05} & 0.02 & {73.71} & {73.56} & 0.00 \\
% GS-LoRA++ \cite{zhao2025practical} &\textbf{1.28\%}& {71.12} & {71.36} & 0.00 & {72.04} & {71.35} & {0.00}  & {71.56} & {68.52} & 0.00 & {72.85} & {71.86} & 0.00 \\ 
% \midrule
% \rowcolor{gray!30} % 设置当前行颜色
% FEAST &\textbf{1.28\%}& \textbf{71.78} & {72.71} & {0.00} & \textbf{72.52} & {72.31} & {0.00}  & \textbf{74.18} & {73.51} & {0.00} & \textbf{75.49} & {77.15} & {0.00} \\ 
% \bottomrule
% \end{tabular}%
% }
% \caption{{Single-step forgetting results for face recognition task on CASIA-Face100.} $Acc_r\ (\%)$ and $Acc_f\ (\%)$ are the accuracies of remaining and forgotten classes.
% $^*$~denotes the original methods with a rehearsal buffer.
% Retrain represents retraining the model using replay data and \textit{the training epoch is the same as other methods to ensure a fair comparison.} Pre-train denotes the results before forgetting.
% All setting is in the form of 100-Y, which means all experiments start from a pre-trained model (100 classes originally) and forget Y classes.}
% \label{tab:single-recog-caisa100}
% \vspace{-0pt}
% \end{table*}



% \begin{table*}[t!]
% \centering
% \vspace{-5pt}
% % \renewcommand{\arraystretch}{1.1}
% % \setlength{\tabcolsep}{6pt}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lrrrrrrrrrrrrrr}
% \toprule
% \multirow{2}{*}{Methods} &\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Tunable\\ Ratio $\downarrow$ \end{tabular}} & \multicolumn{3}{c}{100-5} & \multicolumn{3}{c}{100-10} & \multicolumn{3}{c}{100-50} & \multicolumn{3}{c}{100-90} \\ 
% \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14} 
%  && $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ & $H \uparrow$ & $Acc_r \uparrow$ & $Acc_f \downarrow$ \\ \midrule
% Pre-train & - & - & 73.85 &  70.88& -  & 73.81 & 72.74 & - & 72.45 & 74.88 & - & 72.32 & 73.86 \\
% \midrule
% % \multicolumn{5}{l}{\textcolor{orange}{\textit{(a) continual learning methods}}} \\
% L2$^*$& 99.73\% & 67.13 & 66.96 & 3.58 & 67.74& 64.87&1.86& 64.39 & 56.61 & 0.24 & 52.45 & 40.68 & 0.04  \\
% GS-LoRA \cite{zhao2024continual} &\textbf{1.28\%}& {71.02} & {71.16} & 0.00 & {71.76} & {70.81} & {0.00}  & {71.29} & {68.05} & 0.02 & {73.71} & {73.56} & 0.00 \\
% GS-LoRA++ \cite{zhao2025practical} &\textbf{1.28\%}& {71.12} & {71.36} & 0.00 & {72.04} & {71.35} & {0.00}  & {71.56} & {68.52} & 0.00 & {72.85} & {71.86} & 0.00 \\ 
% \midrule
% \rowcolor{gray!30} % 设置当前行颜色
% FEAST &\textbf{1.28\%}& \textbf{71.78} & {72.71} & {0.00} & \textbf{72.52} & {72.31} & {0.00}  & \textbf{74.18} & {73.51} & {0.00} & \textbf{75.49} & {77.15} & {0.00} \\ 
% \bottomrule
% \end{tabular}%
% }
% \caption{{Single-step forgetting results for face recognition task on CASIA-Face100.} $Acc_r\ (\%)$ and $Acc_f\ (\%)$ are the accuracies of remaining and forgotten classes.
% $^*$~denotes the original methods with a rehearsal buffer.
% Retrain represents retraining the model using replay data and \textit{the training epoch is the same as other methods to ensure a fair comparison.} Pre-train denotes the results before forgetting.
% All setting is in the form of 100-Y, which means all experiments start from a pre-trained model (100 classes originally) and forget Y classes.}
% \label{tab:single-recog-caisa100}
% \vspace{-0pt}
% \end{table*}




% % 4.--1.disentangled feature subspace的构建和相应的disturb-denoise的实现方式
% % Table \ref{tab:subspace}

% % 4.-.lora加在不同的地方，attention or ffn

% % 4.1subspace构建的时候需要 $\epsilon$这个参数对于性能的影响，消融

% % 4.3核范数的设计有什么优势？

% % 讲核范数能够在趋向于正交的同时尽可能使得低秩，因此在forgetting上更有好处，但是在remaining上只需要和补空间正交不需要其他的约束，因此L2 norm已经够了。
% % 给实验结果


% % 4.2continual forgetting on 更多的数据集上和benchmark上

% % 4.3single-step forgetting 
% % 1-99，体现的是我们方法的可扩展性


% % 3.遗忘的恢复效果
% % 在imageNet100上的恢复效果

% % 4.更多的tsne图


% % face上的图
% % 4.1.forget5remain10得图还有7x3张，
% % 7行3列

% % 4.2.大图100类得1张
% % 图太大了，可能需要放到三个页面

% % 4.3要不要加imageNet100的图？？


% % 5.更多的实验结果关于特征还原

% % 5.1提供还原的方法，ae
% % 5.2还原的过程，iteration 
% % 5.3还原的不同层的特征以及对应的psnr和ssim
% % 5.4对于forgetting data和remaining data都进行这一步。要强调的是
% % 对于forgetting data的还原，我们比他们差；对于remaining data的还原，我们比他们好，更加接近于原始特征


